DBO: Response Time Fairness for Cloud-Hosted Financial Exchanges

In this paper, we consider the problem of hosting financial exchanges in the cloud. Financial exchanges require predictable, equal latency to all market participants to ensure fairness for various tasks, such as high speed trading. However, it is extremely difficult to ensure equal latency to all market participants in existing cloud deployments, because of various reasons, such as congestion, and unequal network paths. In this paper, we address the unfairness that stems from lack of determinism in cloud networks. We argue that predictable or bounded latency is not necessary to achieve fairness. Inspired by the use of logical clocks in distributed systems, we present Delivery Based Ordering (DBO), a new approach that ensures fairness by instead correcting for differences in latency to the participants. We evaluate DBO both in our hardware test bed and in a public cloud deployment and demonstrate that it is feasible to achieve guaranteed fairness and sub-100 microsecond latency while operating at high transaction rates.

==> eval_old.tex <==
\section{Evaluation}
\label{s:eval}


We wish to understand how our solution affects fairness and overall latency on a financial-exchange deployment. We also want to better understand the tradeoffs introduced by each mechanism proposed in our system: how does DBO alone improve direct delivery, how do heartbeats affect end-to-end latency, could a `straggler' RB  affect the system's latency etc.
\pg{I think we don't do heartbeats. Maybe add we are most interested in understanding how to performance an latency numbers look like in public cloud. }


\subsection{Methodology}
\label{ss:eval_methodology}


 
For all of the experiments (except simulation) presented in this section we leverage our prototype CES and MP implementations. On the CES side, we generate and distribute data to all Market Participants at fixed intervals. The market data arrive at the RBs, which later on release them to the  Market Participants. The MP implementation relies on busy-polling and kernel-bypass for low-latency access to the incoming market data packets, but does not utilize a sophisticated algorithm for trading decisions; it rather busy-waits for a \eg{random} pre-configured duration (reaction time) before generating a trade. We set each MP's  reaction time accordingly so that we can derive the expected final ordering at the OB and evaluate fairness. 

\noindent\textbf{Fairness metric:} For any number of market participants, perfect fairness is achieved when all competing trades among all unique pairs of participants are fully ordered (from faster to slower). We define the metric of fairness as the ratio of the number of competing trade sets  that were ordered correctly to the total number of competing trade sets for all unique pairs of market participants.

\pg{Note: I use forwarding time instead of execution time}.

\noindent\textbf{End-to-end latency} \pg{Edit: We define end-to-end latency of a trade using Equation~\ref{eq:latency_def} ($F(i,a)-G(x)-RT(i,a)$). Generation time and forwarding time are measured at the CES. For the purpose of reporting latency  and fairness (and not for ordering trades in DBO), we assume that the trigger point is known. We use it to calculate the response time of trades at the release buffer.}

%We define end-to-end latency of any trade, as the duration measured from the market data id transmission (at the CES) until a trade tagged with the same id is executed by the matching engine. This measurement is taken on the CES. 
Our definition of fairness is sufficient for all trades that were generated as a response to some market data within the limited-time horizon, but it could be inaccurate for `slow'  or `non-reactive` trades as they will likely be tagged with a later DBO id. Our solution does not ensure fairness out of the limited horizon, but we explicitly take into account this limitation when presenting latency results in the rest of the experiments.  

 We  evaluate our solution on three different setups: \begin{enumerate*}[label=(\alph*)]\item on-premise, bare-metal testbed deployment, and \item public-cloud-based deployment, \item simulation \end{enumerate*}.

\pg{Evaluation schemes: We evaluate four schemes. \begin{enumerate*}\item Direct delivery: This is the baseline scheme. There is no release buffer or ordering buffer and both trades and market data points just incur the underlying network latency. \item Direct w/ DC: Data is delivered directly to the participants without any batching or pacing. However, the trades are ordered using the delivery clock timestamp. This scheme is used to show the importance of ordering using delivery clocks on its own. \item DBO: We use different values for the horizon ($\delta$) and the batch size($(1+\kappa) \cdot \delta$). \item CloudEx: CloudEx requires fine-grained clock synchronization, which is not available in our test-bed and cloud experiments. Due to inaccuracies in clock-synchronization, in our experiments we experience frequent release buffer and ordering buffer overruns. We only report results for CloudEx in simulation where we assume perfectly synchronized clocks. We also report the optimal latency (max network round-trip-latency Theorem~\ref{thm:latency}) for achieving perfect response time fairness\end{enumerate*}.}

\subsection{Evalution on DPU-enabled baremetal servers}
\label{ss:on-premise-eval}

Our lab setup consists of three machines: one CES server and two MP servers. The CES server is equipped with an Nvidia ConnectX-5 NIC with two 100Gbps ports. Each MP server hosts one Nvidia BlueField-2 DPU with two 100Gbps ports. The server has a dual-CPU Intel Xeon processor running at 3.1 GHz. Each BlueField-2 DPU has eight ARMv8 A72 cores. All machines are connected via a 100GbE switch. We run Linux kernel (v5.4.0) and DPDK (v21.11) for the CES, RB, MP network engines.

The CES is generating market data every $40\mu s$ ($25K$ ticks per second), and the market participant servers are generating responses within $\delta$ time horizon since the reception of the data. The Release Buffer component is executing on the Bluefield-2 DPU's SoC.


Table~\ref{tbl:bluefield} shows the achieved fairness and latency of our system. Delivery clocks based ordering on top of direct delivery significantly enhances fairness, while DBO achieves perfect fairness. \pg{EDIT: Since with both these schemes at the OB we need to wait for the slowest participant, the latency is higher. As explained earlier, waiting for the slowest participant is necessary for achieving fairness.}

\pg{We should explain these results. The next statement seems inconsitent with the results?}
Even though this is a bare-metal, on-premise lab setup with no interfering traffic the tail latency is higher than expected. Our performance analysis indicates that this overhead is due to scheduling artifacts in the Bluefield ARM cores, and higher SoC-to-NIC latencies.\pg{WHAT SHOULD WE SAY ABOUT SOC TO  NIC LATENCY? how are we measuing fairness, what is the response tiem} We are currently working with NVIDIA to utilize their hardware-assisted pacing and NIC timestamping features to improve performance.%\pg{Should we say for calculating fairness ratio we use time stamps taken at the RB? What are the response times?}

\begin{table}[t]
\small
    \centering
    \begin{tabular}{c|c|cccc}
    %\hline
    & \textbf{Fairness} & \multicolumn{4}{c}{\textbf{Latency $(\mu s)$}} \\
    & \textbf{(\%)} & \textbf{avg} & \textbf{p50} & \textbf{p99} & \textbf{p999} \\
    \hline
       \textbf{Direct} & 85.79 & 10.15 & 9.70 & 16.40 & 26.60 \\
       \textbf{Direct w/ DC} &  97.01 & 23.46 & 15.09 & 41.55 & 53.80 \\
       \textbf{DBO (20,25)}  & 100 &  15.92 & 12.16 & 28.82 & 46.80 \\
        \textbf{DBO (45,60)}  & 100 & 28.18 & 20.13 & 64.86 & 94.85  \\
        \textbf{DBO (80,120)}  & 100 & 56.05 & 52.71 & 104.31 & 120.42  \\


    %\hline
    \end{tabular}
    %\vspace{-1mm}
    \caption{\small{Fairness and trade latency results on bare metal servers with BlueField-based RB implementation.} \pg{Something is wrong here, how can latency of direct w/DC be higher than DBO? Can we report max of RTT as well?}}
    \label{tbl:bluefield}
    \vspace{-7mm}
\end{table}




\subsection{Cloud-hosted Testbed}
\label{ss:cloud-eval}



We wish to understand how our system performs in a real public cloud-based deployment with several market participants. As discussed in \ref{ss:release_buffer}, we do not have access to the cloud providers' programmable NICs to deploy the RB functionality. To work around this limitation, we have adjusted our RB implementation so that it runs as a co-located  process with the market participant's execution engine on the MP VMs. In such configuration, the RB is using a kernel-bypass network stack to take over a dedicated vNIC which it uses to receive the UDP stream of market data from the CES, and to send back any trades submitted by the MP. To facilitate fast MP-to-RB communication we rely on shared-memory-based IPC primitives. Clearly, such a solution does not provide any security guarantees, as the RBs run on VMs owned by the market participants which are not part of the CES' Trusted Computing Base, and could easily tamper with the RB's market data delivery engine or the response time measurements. It allows us, however, to evaluate the real-world performance (i.e., achievable throughput and latency) of our DBO system in a public cloud deployment.



\begin{table}[h!]
\small
    \centering
    \begin{tabular}{c|c|cccc}
    %\hline
    & \textbf{Fairness} & \multicolumn{4}{c}{\textbf{Latency $(\mu s)$}} \\
    & \textbf{(\%)} & \textbf{avg} & \textbf{p50} & \textbf{p99} & \textbf{p999} \\
    \hline
       \textbf{Direct} & 57.61 & 27.9 & 27.48 & 32.5 & 44.03 \\
       \textbf{Direct w/ DC} &  89.84 & 47.15 & 47.10 & 57.23 & 312.92 \\
       \textbf{DBO (20,25)}  & 100 &  55.78 & 47.09 & 59.40 & 1366.15 \\
        \textbf{DBO (45,60)}  & 100 & 77.21 & 52.54 & 135.27 & 573.70  \\
        \textbf{DBO (80,120)}  & 100 & 89.32 & 86.89 & 133.23 & 459.97  \\
        \textbf{Max-RTT}  & - & 32.94 & 32.14 & 42.63 & 105.49  \\


    %\hline
    \end{tabular}
    %\vspace{-1mm}
    \caption{\small{Fairness and end-to-end latency results for different schemes.} \pg{Drop p999}}
    \label{tab:fairness_latency}
    \vspace{-7mm}
\end{table}

We set out to evaluate the fairness and end-to-end latency of different schemes. We deploy ten market participants and one Central Exchange Server as virtual machines in Microsoft Azure. We configure the  aggregate service rate to $125,000$ transactions (trades) per second (market data generation interval is fixed to $40\mu s$). Table~\ref{tab:fairness_latency} summarizes the achieved fairness and end-to-end latency results across different schemes. \pg{Can we include a citation here for number of trades?}

\noindent\textbf{Fairness:} Direct delivery achieves poor fairness in our experiments. When combined with DC-based ordering at the OB  fairness is improved significantly. Finally, DBO (regardless of $\delta$) always achieve perfect fairness as all MPs are configured to (randomly) generate trades within the limited horizon. We discuss fairness for slow responders in Section~\ref{ss:simul}.  

\noindent\textbf{Latency:}  As expected, direct delivery achieves  the lowest latency, at the cost of fairness. 
%Direct delivery with Delivery Clock-based ordering, is an enhanced version of direct delivery; as mentioned previously we maintain the delivery clock at the RB and tag each trade received with it, but there is no other delay (pacing, batching etc) introduced at the MP's end. Instead,  the OB sorts all trades based on their DC-derived timestamp and forwards them to the ME when it has heard from all RBs. In practice, this means that the  end-to-end latency for all MPs is effectively \textit{inflated} to the worst CES-to-MP network RTT experienced.
As discussed, DBO trades off latency to achieve perfect fairness. In particular, the latency is bounded by maximum network round-trip latency. 
Batching and pacing further add to this optimal latency. We see that increasing $\delta$, increases the latency. When the network is well behaved this increase is linear. However, we find that 

%When the network is well behaved, the end-to-end latency is similar to that of direct delivery with DC-based ordering which constitutes optimal for DBO. %The increased tail latency results presented here are due to OS scheduling artifacts and network events such as possible heartbeat drops or RTT spikes. 
%\im{I am handwaiving here and i don't like it} 

\subsubsection{Understanding DBO latency:}

\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{images/latency_cdf_bf2.png}
    % \includegraphics[width=0.95\columnwidth]{images/latency_cdfs2.pdf}
    \caption{\small{\bf CDFs of the end-to-end trade latency for various DBO configurations on bare metal servers with BlueField-based RB implementation. \pg{we need comparison with direct delivery here. And fairness numbers}}}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{images/latency_cdfs.pdf}
    % \includegraphics[width=0.95\columnwidth]{images/latency_cdfs2.pdf}
    \caption{\small{\bf CDFs of the end-to-end trade  latency for various DBO configurations. Max-RTT CDF corresponds to the highest network RTT among all participants.}}
    \label{fig:latency_cdfs}
\end{figure}

How does batching and pacing affect end-to-end trade latency? Figure~\ref{fig:latency_cdfs} illustrates the latency with different DBO configurations. 

\im{I don't think we have space for that, and I don't understand why MaxRTT CDF does not match DBO(20,25)}



\subsubsection{Impact of straggler RBs}

\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{images/straggler_mitigation.pdf}
    \caption{\small{\bf Stragglers' impact to end-to-end trade  latency for all market participants. }}
    \label{fig:straggler_mitigation}
\end{figure}

At this point, it is important to differentiate a straggler RB from slow MP responders: the RB is part of the Trusted Computing Base and hence correct operation is critical for good end-to-end system performance. Still, failures and non-determinism stemming from the network need to be taken into account in our system design. 

A straggler RB (i.e., experiencing high latencies or packet drops) can drastically affect the end-to-end system latency and throughput. This happens because the OB needs to hear from all RBs before dequeuing trades to the matching engine, so that fairness is guaranteed. In Figure~\ref{fig:straggler_mitigation} we evaluate how latency is affected with a straggler; we emulate this by configuring one of the RBs to drop all packets (including outgoing hearbeats) as would happen in the case of a transient network outage. Such events could potentially stall to the market indefinitely; to mitigate this issue the OB maintains a timeout (in this case set to 250us) and on expiration releases trades for the current DBO id to the ME. In such cases, fairness guarantees do no longer hold for the straggler.

A production deployment should leverage a mechanism to detect and flag stragglers quickly; upon detection, straggler RBs should be removed from the OB's shard so that the market does not unnecessarily  slow down for prolonged periods.

\subsection{Latency overhead with multiple participants}

DBO \textit{post} corrects for latency variance at the OB. As the number of market participants increases, network RTT variance and asynchrony might be pronounced and can cause higher delays at the Ordering Buffer. In Figure~\ref{fig:ob_delay} we plot the time spent at the OB as a function of the market participants. Note, that the RB components remain unaffected as the number of participants gets higher.


\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{images/ob_delay_boxplot2.pdf}
    \caption{\small{\bf Trades' buffering delay at the Ordering Buffer. \im{make this figure smaller.}}}
    \label{fig:ob_delay}
\end{figure}





\subsection{Simulation}
\label{ss:simul}

We evaluate fairness and end-to-end latency of DBO as a function of the number of market participants in simulation, and we compare against Cloudex and direct delivery schemes.

Figure~\ref{subfig:fairness} shows the fairness achieved by each scheme. In our simulation, we have modelled network RTTs to follow a .... distribution and market participants' to generate trades within (0, $\delta$)us since the market data reception. DBO achieves 100\% latency regardless of the number of market participants. 



\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{images/simulation_latency.pdf}
    \caption{\small{\bf Network trace used in simulation.}}
    \label{fig:sim_trace}
\end{figure}


\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{images/sim_part_fairness.pdf}
    \vspace{-5.5mm}
    \caption{\small{Fairness}}% ($C_{S1}=1.14$, $\delta=14\mu s$)}%Strategy S1 with $C_{S1}=1.14$, $\delta=14\mu s$}
    \label{subfig:fairness}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{images/sim_part_avg_latency.pdf}
    \vspace{-5.5mm}
    \caption{\small{Mean Latency}}% ($C_{S2}=1.1$)}%Strategy S2 with $C_{S2}=1.2$}
    \label{subfig:mean_latency}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\linewidth}
    %\includegraphics[width=\linewidth]{images/ARTF-2.pdf}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{images/sim_part_tail_latency.pdf}
    \vspace{-5.5mm}
    \caption{\small{Tail Latency}}
    \label{subfig:tail_latency}
  \end{subfigure}
  \vspace{-3mm}
  \caption{\small{\textbf{Fairness and Latency trends with number of participants.}.}}% Except CloudEx, all other schemes used DBO.}% \pg{I wonder if we should the extend the x-axis to 64 or 128 $\mu s$. The point would be too show that all schemes can achieve reasonable performance when response times are high, it is hard when they are low.}}
  \vspace{-4.5mm}
  \label{fig:sim_participant}
\end{figure*}



\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{images/sim_delta.pdf}
    \caption{\small{\bf Fairness beyond LRTF: Using clocksync with DBO.}}
    \label{fig:sim_delta}
\end{figure}


==> hotnets/abstract.tex <==
%\pg{Ilias's attempt
%\vspace{-20mm}

 

%\im{work in progress, shorten it as much as possible} 
%\pg{Work in progress} Despite significant advancements in cloud computing technology in recent years, some workloads remain unsuitable for the cloud.
%Currently, financial market infrastructure is housed in on-premise data centers. There are several reasons that encourage the move of important financial market services to the public cloud, including elastic resource scalability and significant cost savings. Moving the financial ecosystem to the cloud, on the other hand, necessitates overcoming considerable difficulties and potentially adopting a new operational paradigm. 
%The  operation of modern financial exchange servers relies on predictably equal and low latency for all market transactions: cloud networks, however, were not initially designed to retain such features, particularly affecting fairness for all market participants.
%The  operation of modern financial exchange servers relies on predictability, low latency, and fairness for all market transactions: cloud networks, however, were not initially designed to retain such features, particularly affecting fairness for market participants. %\pg{What do you mean by predictability?}

%In this paper, we attempt to solve the problem of unfairness that stems from the lack of determinism in contemporary cloud networks. We show that predictable %latency is not necessary to achieve fairness, and we present a few scalable strategies that yield \im{good, perfect, satisfactory} fairness while incrementally %deployable in contemporary cloud environments. Our system outperforms the current state-of-the-art in simulation \im{by XX\%} while at the same time avoiding %critical limitations.  \pg{I dont like the last two lines can we just leave it at we explore the use of logical clocks for fairness.} 

%In this paper, we consider the problem of supporting modern financial exchange services on the cloud premises. Important financial exchange services rely on predictable, equal latency from the servers to the participants for fairness. Contemporary cloud networks, however, are unable to offer such property, as they were not originally designed for this purpose. We attempt to tackle the problem of unfairness that stems from the lack of determinism in contemporary cloud networks. We argue that predictable latency is not necessary to achieve fairness, and we propose a novel approach that is deployable in contemporary cloud environments. We evaluate our approach in simulation and we show how it is feasible to achieve fairness even under unbounded and fluctuating network latency.  Our approach avoids limitations of state-of-the-art and outperforms it.% by a factor of X\%.  

%\attn{In this paper, we consider the problem of supporting modern financial exchange services on the cloud premises. Important exchange services rely on predictable, equal latency from the servers to the participants for fairness. Existing cloud networks, however, are unable to offer such property, as they were not originally designed for this purpose. We attempt to tackle the problem of unfairness that stems from the lack of determinism in cloud networks. We argue that predictable or bounded latency is not necessary to achieve fairness. Inspired by the use of logical clocks in distributed systems, we propose a new approach that is deployable in contemporary cloud environments. We evaluate our approach in simulation and show that it is feasible to achieve fairness under highly variable network latency. Our approach avoids limitations of state-of-the-art and outperforms it.}

\attn{In this paper, we consider the problem of supporting modern financial exchange services on the cloud premises. Important exchange services rely on predictable, equal latency from the servers to the participants for fair competition. Existing cloud networks, however, are unable to offer such property, as they were not originally designed for this purpose. We attempt to tackle the problem of unfairness that stems from the lack of determinism in cloud networks. We argue that predictable or bounded latency is not necessary to achieve fairness. Inspired by the use of logical clocks in distributed systems, we propose a new approach that instead corrects for differences in latency to the participants for fairness. We evaluate our approach in simulation and show that it is feasible to achieve fairness under highly variable network latency. Our approach is deployable in contemporary cloud environments; it avoids limitations of state-of-the-art and outperforms it.}

% eg{Financial exchanges are an integral part of the capital market. In this paper, we consider the problem of unfairness caused by the nondeterminism of cloud networks and propose a solution to maintain temporal fairness for financial exchanges. Inspired by the use of logical clocks, }

==> hotnets/achieving_prateesh.tex <==
%\section{Using the tool-kit}
%\section{Evaluation}
\section{Achieving Fairness}%\pg{better title?}}
\label{s:exp}

%\pg{Should we include both S2 and S3? I chose S2 because it provide some contrast over the cloudEx soltuin. S3 I included just because I think its a reasonable scheme.}
%Based on Section \ref{s:core}, as long as the time span between consecutive deliveries of market data (inter-delivery time) to the MPs satisfy the required constraints, we can guarantee the corresponding type of fairness in trade handling at the CES. Based on these constraints, we introduce a few fairness algorithms and later compare them against the Cloudex.

In the previous section, we derived the minimum constraints on the delivery processes for achieving different variants of fairness. In each case, we also showed that if these constraints are met, then, DBO achieves fairness. Which property/properties for the delivery process should the cloud-provider aim for and what is the best way to achieve them (with low latency and high probability) depends on many things, including the requirements for fairness of the financial exchange and the nature of latency variations in the cloud-provider. In this paper, we do not attempt to provide any verdict on this question. Instead, in this section we only aim to show that DBO coupled with controlling how delivery clocks advance can indeed provide fairness with high probability in scenarios where the network latency is highly variable. To this end, we propose two simple schemes (with very different trade-offs for fairness) for delivering market data that both use DBO for ordering trades. We also compare these schemes against CloudEx. %($D_i(x) = \max(R_i(x), G_i(x)+Th)$) and $O(i,k) =A_i(k)$).}
%where the data is delivered at the same time to all MPs ($D_i(x) = \max(R_i(x), G_i(x)+Th)$) and trades are ordered based on the submission time ($A_i(k)$).}

\begin{figure}[t]
    \centering
    \includegraphics[trim={0 0 0 0mm},clip,width=\linewidth]{hotnets-images/latency_map_alt.pdf}
    \vspace{-6mm}
    \caption{\small{\textbf{Visualizing delivery times:} x-axis shows the generation time of the market data. y-axis plots the delivery times relative to the generation time for market data points (i.e., $D_i(x)-G(x)$) for different schemes. We also include the latency from the CES to the MP for reference (dotted black line). The dashed vertical lines demarcate various regions of interest for scheme S2.}}
    %\pg{Eashan: Include the drain rate, make the colored lines thicker and use different linestyles for the three schemes..}}% \pg{Maybe label the drain rate in the figure for S1 and S2.}}
    \label{fig:latency_graph}
    \vspace{-5mm}
\end{figure}

To help understand these two schemes, we consider a simple scenario where the latency from the CES to a single MP is mostly constant except a transient spike. \Fig{latency_graph} depicts the delivery times of each of the two schemes for this particular MP.

%To help you visualize, \Fig{latency_graph} shows the delivery times for each scheme for a particular MP in a simple scenario. The latency from CES to the MP is constant except a transient spike.

\smallskip
\noindent
\textit{Scheme 1 (S1):} The inter-delivery times respect the constraints in Corollary~\ref{cor:1} and S1 provides limited fairness regardless of the variations in network latency. In S1, the CES splits the market data points into batches. %The CES includes the corresponding batch number for each market data point.
At the RB, all the market data points corresponding to the same batch are delivered simultaneously (i.e., the inter-delivery time for market data points within a batch is zero). The time interval between delivery of two batches is greater than or equal to $\delta$. \attn{Note that, as per Corollary~\ref{cor:1}, the inter-batch time at a MP can differ from other MPs. As a result, S1 can handle arbitrary latency spikes without violating the inter-delivery constraints.} %In the event of a latency spike, a RB can delay delivering the next batch arbitrarily. As a result, S1 can handle arbitrary latency spikes without violating the inter-delivery constraints.} 
%As a result, S1 can handle arbitrary latency spikes, In the event of a latency spike RB can delay the next batch arbitrarily. Thu without violating the inter-delivery constraints. } 
Formally, delivery time of a batch $b$, ($D_i(b)$), is given by,
\begin{align*}
    D_i(b) = \max(R_i(b), D_i(b-1)+\delta),
\end{align*}
where $R_i(b)$ is the time  at which the last market data point in $b$ is received by RB$_i$. The CES chooses the batch boundaries based on the generation time of the market data. Market data $x$ corresponds to batch number ($b(x)$) given by $b(x) = \lfloor\frac{G(x)}{C_{S1}\cdot\delta}\rfloor$ or equivalently $C_{S1}\cdot\delta \cdot b(x) \leq G(x) < C_{S1}\cdot\delta \cdot (b(x)+1)$, where $C_{S1} (> 1)$ is a constant. \attn{Note that, with S1 batches can be arbitrarily small and multiple batches can be outstanding within a round trip.}

% \eg{\textit{Scheme 1 (S1):} The inter-delivery times respect the constraints in Corollary~\ref{cor:1} and S1 provides limited fairness regardless of the variations in network latency. In S1, the market data points are delivered in batches, with all the market data points corresponding to the same batch delivered simultaneously . the RB waits for all points in a batch to be rceived from the CES before transmitting the complete batch to the MP batches are delivered as soon as all data points of the said batch are received  a minimum \attn{Note that, as per Corollary~\ref{cor:1}, the inter-batch time at a MP can differ from other MPs. As a result, S1 can handle arbitrary latency spikes without violating the inter-delivery constraints.} Formally, delivery time of a batch $b$, ($D_i(b)$), is given by,
% \begin{align*}
%     D_i(b) = \max(R_i(b), D_i(b-1)+\delta),
% \end{align*}
% where $R_i(b)$ is the time  at which the last market data point in $b$ is received by RB$_i$. The CES chooses the batch boundaries based on the generation time of the market data. Market data $x$ corresponds to batch number ($b(x)$) given by $b(x) = \lfloor\frac{G(x)}{C_{S1}\cdot\delta}\rfloor$ or equivalently $C_{S1}\cdot\delta \cdot b(x) \leq G(x) < C_{S1}\cdot\delta \cdot (b(x)+1)$, where $C_{S1} (> 1)$ is a constant. \attn{Note that, with S1 batches can be arbitrarily small and multiple batches can be outstanding within a round trip.}}

%\pg{Explain C?} 
%\attn{Note that ~\cite{frequent_batch_auctions} also proposes delivering market data in batches. However unlike S1, it aims for all trade orders corresponding to a batch to be processed at the CES first before the next batch is released. To this end, it uses big batch sizes ($\sim$ 100 ms) that introduces significant latency. In contrast, with S1 the batches can be arbitrarily small and multiple batches can be outstanding within a round trip.}
 
\smallskip
\noindent
\textit{Scheme 2 (S2):} For this scheme, we assume clock synchronization between RBs. The mechanism for data delivery is an extension over CloudEx based on the constraints in the previous section. Formally,
\begin{align*}
    D_i(x) = \max\left(R_i(x), G(x)+Th, D_i(x-1) + \frac{G(x)-G(x-1)}{C_{S2}}\right)
\end{align*}
where $C_{S2} (> 1)$ is a constant. Intuitively, if the network latencies for all the MPs are below $Th$ consistently (region \circled{1} and \circled{4} in \Fig{latency_graph}), then, the inter-delivery time at each MP is the same (equal to the inter-generation time, i.e., $D_i(x)-D_i(x-1)= G(x)-G(x-1), \forall i$). The delivery times thus respect the constraints in Theorem~\ref{thm:1} and S2 provides strong fairness at such times. Compared to CloudEx, the main differentiation of the scheme above is how data delivery is handled after a latency spike between the CES and a particular MP (third term in the equation). In such cases (region \circled{3}), the inter-delivery time differs from the inter-generation time by a relative factor ($C_{S2}$) and $D_i(x)-D_i(x-1)= \frac{G(x)-G(x-1)}{C_{S2}}$. At such times, if the network latency to other MPs remains consistently low, then the inter-delivery time gaps respect the constraints listed in Corollary~\ref{cor:2} (with $\epsilon = C_{S2} - 1$) and $S2$ provides approximate fairness.%, at the cost of some additional latency compared to CloudEx. 
The inter-delivery time gaps at MPs, however,  can differ significantly when latency spikes happen (region \circled{2}), hence leading to reduced fairness by S2. Despite this, since S2 uses DBO, it can still correct for late delivery of market data and provide better fairness than CloudEx in such cases. 

Note that, it is equally possible to achieve the above inter-delivery properties without clock-sync. We chose S2 specifically to show incremental benefits over CloudEx from incorporating DBO and trying to respect the constraints on inter-delivery times.


% \textit{Scheme 2 (S2):} For this scheme, we assume clock synchronization between RBs. The mechanism for data delivery is a simple extension over CloudEx based on the constraints in the previous section. Formally,
% \begin{align*}
%     D_i(x) = \max\left(R_i(x), G(x)+Th, D_i(x-1) + \frac{G(x)-G(x-1)}{C_{S2}}\right)
% \end{align*}
% where $C_{S2} (> 1)$ is a constant. Intuitively, if the network latencies for all the MPs are as expected and below $Th$ (regions \circled{1} and \circled{4} in \Fig{latency_graph}), then, the inter-delivery time at each MP is the same (equal to the inter-generation time, i.e., $D_i(x)-D_i(x-1)= G(x)-G(x-1), \forall i$). The delivery times thus respect the constraints in Theorem~\ref{thm:1} and S2 provides strong fairness at such times. In the case of a sudden latency spike between CES and a particular RB (region \circled{2}), we follow a best effort approach (first term in the equation). In such a case, the inter-delivery times across MPs would differ leading to reduced fairness. The main difference in S2 as compared to Cloudex is how it provides fairness after the spike (region \circled{3}). In such cases, the inter-delivery time differs from the inter-generation time by a relative factor $C_{S2}$ (third term of the equation) and $D_i(x)-D_i(x-1)= \frac{G(x)-G(x-1)}{C_{S2}}$. At such times, if the network latency to other MPs remains consistently low, then the inter-delivery time gaps respect the constraints listed in Corollary~\ref{cor:2} (with $\epsilon = C_{S2} - 1$) and $S2$ provides approximate fairness.


%\pg{Even in this case because of DBO S2 is better than cloudex}


\begin{figure}[t]
    \centering
    \includegraphics[trim={0 0 0 5mm},clip,width=0.9\linewidth]{hotnets-images/transmission_times.pdf}
    \vspace{-4mm}
    \caption{\small{\textbf{Variations in latency from the CES to the RBs.}}} %\pg{Eashan You can shrink the height further, in the legend use ncol=2}} %\pg{Eashan can you redeaw this figure so that the height is smaller. Increase tick label size and legend size.}
    \label{fig:transmission_times}
    \vspace{-5mm}
\end{figure}

% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{images/LRTF delivery.pdf}
%     \caption{S1}% ($C_{S1}=1.14$, $\delta=14\mu s$)}%Strategy S1 with $C_{S1}=1.14$, $\delta=14\mu s$}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.31\linewidth}
%     \includegraphics[width=\linewidth]{images/ARTF.pdf}
%     \caption{S2}% ($C_{S2}=1.1$)}%Strategy S2 with $C_{S2}=1.2$}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.36\linewidth}
%     \includegraphics[width=\linewidth]{images/clocksync.pdf}
%     \caption{Cloudex}% ($d_o=300, d_i=100$)}%we describe them already
%   \end{subfigure}
%   \vspace{-5mm}
%   \caption{\textbf{Fairness with different schemes.} Fraction of trades that were ordered fairly for different values of response time.}
%   \vspace{-3mm}
%   \label{fig:fairness-sim}
% \end{figure*}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.245\linewidth}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{hotnets-images/clocksync.pdf}
    \vspace{-5.5mm}
    \caption{\small{Cloudex}}% ($C_{S1}=1.14$, $\delta=14\mu s$)}%Strategy S1 with $C_{S1}=1.14$, $\delta=14\mu s$}
  \end{subfigure}
  \begin{subfigure}[b]{0.23\linewidth}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{hotnets-images/LRTF delivery.pdf}
    \vspace{-5.5mm}
    \caption{\small{S1 (Batch delivery + DBO)}}% ($C_{S2}=1.1$)}%Strategy S2 with $C_{S2}=1.2$}
  \end{subfigure}
  \begin{subfigure}[b]{0.23\linewidth}
    %\includegraphics[width=\linewidth]{images/ARTF-2.pdf}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{hotnets-images/ARTF.pdf}
    \vspace{-5.5mm}
    \caption{\small{S2 (CloudEx$^+$ deli + DBO)}}
  \end{subfigure}
  \begin{subfigure}[b]{0.264\linewidth}
    \includegraphics[trim={0 0 0 1mm},clip,width=\linewidth]{hotnets-images/Cloudex delivery+DBO.pdf}
    \vspace{-5.5mm}
    \caption{\small{S3 (CloudEx delivery + DBO)}}% ($d_o=300, d_i=100$)}%we describe them already
  \end{subfigure}
  \vspace{-3mm}
  \caption{\small{\textbf{Fairness with different schemes.} Fraction of trades that were ordered fairly for different values of response time. 
  Closer to 1 (white) is better.}}% Except CloudEx, all other schemes used DBO.}% \pg{I wonder if we should the extend the x-axis to 64 or 128 $\mu s$. The point would be too show that all schemes can achieve reasonable performance when response times are high, it is hard when they are low.}}
  \vspace{-4.5mm}
  \label{fig:fairness-sim}
\end{figure*}


\pg{This is more fundamental move to the core section}
\smallskip
\noindent
%\textit{Buffering algorithm at the OB:} 
\textit{Handling latency variations on the reverse path:} 
The latency from the MPs to the CES could also be variable. Such variations do not affect fairness as long as the OB only forwards a trade $(i,k)$ to the ME once it has (received and) forwarded all other trades $(j,l)$ that should be ordered ahead of $(i,k)$ (i.e., $O(j,l) < O(i,k)$). This requirement means that the OB might need to delay received trades for a certain duration (buffering) before forwarding them to the ME. There are multiple ways to achieve this requirement; we describe a simple one here. Each RB sends an acknowledgement (ACK) for every market data point it delivers to the MP. We assume that ACKs and trades from each RB are delivered to the OB in-order. %using a reliable delivery transport such as TCP. 
An ACK from RB$_j$ for data $x$ thus tells the OB that it has received all trades $(j,l)$ from $MP_j$ s.t., $O(j,l) \leq \langle x, 0 \rangle$. The OB uses a priority-queue to buffer trades. The OB uses the ACK information to forward trades respecting the above requirement. In the event of RB failures, the OB could stall indefinitely waiting for ACKs from a failed RB; we can protect against such scenarios by introducing a timeout threshold. \attn{This timeout can also help reduce buffering at the OB (at the cost of fairness) when the network latency from/to certain MPs is high.}

%In the event of RB failures, the OB could stall indefinitely waiting for ACKs from a failed RB; we can protect against such scenarios by introducing a timeout threshold.

%\eg{This part about in-order and reliable communication seems to have been covered in \S\ref{s:background}:Communication model.}%A trade $(i,k)$ at the head of the queue is forwarded to the ME if the OB has 
%\pg{should we add the following note: in the event of failures, the OB might not receive ACKs from a particular RB and the OB might stall indefinitely. We propose waiting for ACKs only upto a limited time to ward off against such scenarios.}
%Each RB includes a sequence number for the 

 
%\noindent
%\textit{Setup}: Based on the properties, we have the following high level setup: CES generates data point $x$ at local time $t^{\text{CES}}_g(x)$ and multicasts it to all RBs. $\text{RB}_i$ receives $x$ at local time $t^i_r(x)$ and delivers it to $\text{MP}_i$ at $t^i_d(x)$. After delivering the latest data $x$ to the MP, $\text{RB}_i$ marks its current state, $c^i$, as $x$ and $t^i_c=t^i_d(x)$. The $\text{RB}_i$ receives a trade $k$ from $\text{MP}_i$ at local time $t^i_k$ which is transmitted to the CES along with the current state of the $\text{RB}_i$ and the time difference: $<c^i, t^i_k-t^i_c>$. Following the idea of fairness, the CES orders the trades lexicographically based on state of RB when trade was received and the time difference, $<c, t_k-t_c>$. The execution for trade can be carried out once all RBs have reached state $c+1$ which can be ensured by sending out heartbeat messages from RBs to CES or sending ACKS on delivering market data to the MPs.

%Following the above setup, a fairness algorithm can be defined by when $\text{RB}_i$ delivers the market data $x$ to the $\text{MP}_i$ i.e., its policy to determine $t^i_d(x)$. The following fairness algorithms describe the method of market data delivery from the RBs to the MPs.

% \begin{algorithm}
% \floatname{algorithm}{}
% \renewcommand{\thealgorithm}{}
% \caption{RB$_i$}
% \textbf{Receive data $x$ at local time $t^i_r$}
% \begin{algorithmic}
%     \STATE Deliver to MP at time $t^i_d$
%     \STATE Send ACK $x$ to CES
%     \STATE RB$_i$ reached state $x$. Mark current state $c=x$.
% \end{algorithmic}

% \textbf{Receive trade $P$ from MP at $t^i_P$}
% \begin{algorithmic}
%     \STATE Send to CES $(P, <c, t^i_P-t^i_c>)$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \floatname{algorithm}{}
% \renewcommand{\thealgorithm}{}
% \caption{CES}
% \textbf{On generation of data $x$ at} $t^{\text{CES}}_x$\textbf{, multicast $x$ to all RBs}\\
% \textbf{On receiving trade from RB$_i$: $(P, <x_l, t_P-t_c>)$}
% \begin{algorithmic}
%     \STATE Wait until all RBs have reached state $(x+1)$
%     \STATE Execute $P$ based on the ordering
% \end{algorithmic}

% \textbf{Receive ACK $x$ from RB$_i$}
% \begin{algorithmic}
%     \STATE Mark RB$_i$ as having reached $x$
% \end{algorithmic}
% \end{algorithm}

%\textbf{Algorithm 1} (Limited Fairness): The data is delivered in batches. RBs wait to collect a complete batch of market data points from the CES and deliver them at once to the MP. This is done while ensuring, with best effort, that the delivery time between batches is exactly $\delta$. The choice of batch size and $\delta$ is such that the queue of market data is drained eventually. Note that following Corollary \ref{cor:1}, this algorithm ensures limited fairness from Section \ref{ss:limited_fairness}.

%\textbf{Algorithm 2} (Approximate Fairness):  Following Corollary \ref{cor:2}, the data points are delivered based on $t^i_d(x)=t^i_d(x-1)+\frac{1}{1+\epsilon}\cdot(t^\text{CES}_g(x)-t^\text{CES}_g(x-1))$ for some predetermined $\epsilon$. This is again followed with best effort. For this instance, we also assume clock synchrony between all RBs and CES and add a delivery time delay, similar to Cloudex, for which the RBs wait additionally from the point of generation.



%Figure \ref{fig:latency_graph} shows how the discussed algorithms and Cloudex handle a spike in network transmission time between CES and an RB. Cloudex waits for the delay threshold time from the point of generation before delivering the data. Algorithm 1 collects a batch of data, thus has spikes on the initial entries of the batch and delivers them altogether. Algorithm 2 initially works similar to Cloudex but in case of a latency spike, it slowly adjusts back to the delay threshold set.

\subsection{Simulation Results}
\label{ss:simulation}




\if 0
\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.24\linewidth}
    \includegraphics[width=\linewidth]{images/alternate/LRTF delivery.pdf}
    \vspace{-5mm}
    \caption{S1}% ($C_{S1}=1.14$, $\delta=14\mu s$)}%Strategy S1 with $C_{S1}=1.14$, $\delta=14\mu s$}
  \end{subfigure}
  \begin{subfigure}[b]{0.23\linewidth}
    \includegraphics[width=\linewidth]{images/alternate/ARTF.pdf}
    \vspace{-5mm}
    \caption{S2}% ($C_{S2}=1.1$)}%Strategy S2 with $C_{S2}=1.2$}
  \end{subfigure}
  \begin{subfigure}[b]{0.23\linewidth}
    \includegraphics[width=\linewidth]{images/alternate/ARTF-2.pdf}
    \vspace{-5mm}
    \caption{S3}
  \end{subfigure}
  \begin{subfigure}[b]{0.27\linewidth}
    \includegraphics[width=\linewidth]{images/alternate/clocksync.pdf}
    \vspace{-5mm}
    \caption{Cloudex}% ($d_o=300, d_i=100$)}%we describe them already
  \end{subfigure}
  \vspace{-3mm}
  \caption{\textbf{Fairness with different schemes.} Fraction of trades that were ordered fairly for different values of response time. \pg{I wonder if we should the extend the x-axis to 64 or 128 $\mu s$. The point would be too show that all schemes can achieve reasonable performance when response times are high, it is hard when they are low.} \eg{Added results with longer response time to address the concern of RTF schemes only working for HFTs or smaller horizon. We can say that it provides fairness in all scenarios. We can edit and keep the results that are more useful.}}
  \vspace{-3mm}
  \label{fig:fairness-sim-long-rt}
\end{figure*}
\fi
%\pg{Include a note on that we pick static threshold for CloudEx}

To evaluate the proposed schemes, we run a simulation experiment using two dummy MPs with \emph{highly} variable latency between the CES and each RB (generated by a random-walk-like process); see \Fig{transmission_times}. In CloudEx, latency on the reverse path can cause additional unfairness (which can be alleviated using the buffering process we describe earlier). For simplicity, the latency between each RB and the CES is assumed to be fixed (100 $\mu s$). The CES generates market data continuously every $2 \mu s$. We assume that both MPs submit a trade in response to every market data point. We do several runs of the experiment with different values of response times for each MP (fixed across data points within a run). For MP2, we vary the response time ($rt_2$) from 2 to 32 $\mu s$.\footnote{We specifically choose to evaluate over such short response times. For long response times (> 1 ms), all schemes provide close to ideal fairness.} For each value of $rt_2$, we run the experiment such that response time of MP1 ($rt_1$) is higher than from $rt_2$ by some multiplicative factor ($rt_1 = f \cdot rt_2$). We vary $f$ from 1.1 to 2. 





%\textit{Fairness}: 

To measure fairness, we calculate the fraction of MP2's trades that were executed before the corresponding ones (based on the same market data) from MP1. %Following Definition \ref{def:strong}, this fraction would be 1 for an ideal scheme. 
\Fig{fairness-sim}, shows the results for the three schemes.
%Figure \ref{fig:fairness-sim}, shows the fraction of trades that satisfy strong fairness (Definition \ref{def:strong}) for S1, S2 and CloudEx.% in each case. %We construct a heat map to contrast the differences.
We also compare the average end-to-end latency\footnote{The round trip latency between market data generation and trade handling excluding the response time.} (measured across trades) for these schemes (see Table~\ref{tab:latency}). 

%Formally, if a trade $(i,k)$ generated in response to data point $x$, is forwarded to the ME at time $t$, its end-to-end latency is given by $t-(G(x)+rt_i(k))$.  Intuitively, we are measuring the round trip latency between market data generation and trade handling excluding the response time.% of the MP.% to respond to the RB.

$Th$ governs the trade-off between fairness and latency in CloudEx, here we use a fixed $Th = 300\mu s$ s.t., the network latency from CES to the MP is below this threshold most of the time.
For S1, we use a small value of $\delta = 14\mu s$. %$C_{S1}$ governs the buffer drain rate at the RB after a spike and hence the latency.
We chose $C_{S1} \cdot \delta = 16$ s.t., the latency is similar/lower to CloudEx.  For S2, we use $C_{S2} = 1.095$ (< 1.1) to try to ensure the constraint from Corollary~\ref{cor:2} for $\epsilon = 0.095$\footnote{If this constraint is met at all times, then, S2 will achieve ideal fairness when $rt_1 > rt_2*1.095$}. 
We use the same $Th$ as CloudEx to equalize latency.% and to show improvements from DBO and controlling the inter-delivery times. %\pg{I wonder if we should show results pick a higher value of $C_{S2}$ s.t., the last row in heatmap looks bad.}

%\pg{Not sure we should include S3} We also consider another DBO based scheme (S3) here. In S3, each RB tries to maintain a constant amount of market data buffered at the RB. If the buffering goes below a certain threshold, the RB increases the inter-delivery times (by a multiplicative factor ($C_{S3}$) relative to the inter-generation time, $D_i(x) - D_i(x-1) = C_{S3}\cdot(G(x)-G(x-1))$). 
%If the buffering increases, the RB reduces the inter-delivery times ($D_i(x) - D_i(x-1) = \frac{G(x)-G(x-1)}{C_{S3}}$). This scheme ensures that inter-delivery times meet the constraints in Corollary~\ref{cor:2} (with $\epsilon=C_{S3}^{2}-1$) if all RBs have some market data buffered. However, unlike S2, this scheme does not rely on clock synchronization. We use $C_{S3}=\sqrt(1.095)$ and 50$\mu s$ of buffering threshold (to equalize latency).  






As expected, S1 achieves perfect fairness when $rt_2 < \delta$. When the response time is higher, S1 achieves the worst fairness. It is possible to provide better fairness for such trades by additionally trying to ensure that inter-batch delivery times are similar across MPs. 

 S2 provides close to ideal fairness at the cost of some additional latency.\footnote{Fairness with S2 drops when $rt_1 \leq rt_2*1.095$, but it is still comparable to CloudEx.} As explained earlier, this is because the combination of DBO and controlling how delivery clocks advance enables S2 to handle latency spikes better than CloudEx. To understand where the wins in S2 are coming from, we consider another scheme. S3 uses DBO and market data delivery is same as CloudEx. DBO on its own helps correct for differences in latency to the MPs and provides better fairness than CloudEx. By controlling the delivery clocks, S2 is further able to %mask the impact of latency spikes and 
 improve fairness.% than S3.  
 
%Note that, the aim of this experiment is to illustrate the benefits of our approach in scenarios where network latency is highly variable. The exact performance numbers do depend on the latency traces. We repeated the above experiment with other latency traces. In each case, the trend in performance was similar.
 %S2 outperforms S3 by controlling the delivery clocks.  


%\pg{I wonder if we should include an experiment with CloudEx like delivery but with DBO ordering. The point would be too show DBO in its self is useful but you combine it with controlling the delivery clock (S2) it is more useful.}
%Note that even if we increase $Th$ to $300\mu s$ for CloudEx, it still provides worse fairness than S2 (with $Th =250 \mu s$) and its latency is higher than S2.

%\pg{Not sure if we should include S3:} In S3, RBs rarely run out of market data buffering in this experiment. S3 also achieves close to ideal fairness (for similar latencies). Additionally, we can use more sophisticated schemes for managing buffers (e.g., a PID controller~\cite{somepidbook}) to achieve even better performance.


\vspace{-2mm}
\begin{table}[h!]
\small
    \centering
    \begin{tabular}{cc}
    %\hline
        \textbf{Scheme} & \textbf{End-to-end Latency ($\mu s$)} \\
    \hline
        CloudEx & 403 \\
        S1 & 382 \\
        S2 & 408 \\
        S3 & 406 \\
    %\hline
    \end{tabular}
    \vspace{-1mm}
    \caption{\small{End-to-end latency for different schemes.}}
    \label{tab:latency}
    \vspace{-5mm}
\end{table}








==> hotnets/background.tex <==
\section{Background}
\label{s:background}

\subsection{High-level Architecture}
\label{ss:basic_architecture}

%Our system is composed by three discrete entities: the Central Exchange Server (CES), the Release Buffer Components (RBs), and the Market Participants (MPs). The Central Exchange Server is essential component, responsible for serving trade orders.
\Fig{basic_architecture} shows the main components of our system. This architecture is roughly in line with earlier works~\cite{cloudex, libra}. 
%
%
For now, we will assume that each MP is a single machine (or a virtual machine) in the cloud. We will relax this constraint in \S\ref{ss:multi_machine}. 

%\chaitanya{There are broadly two types of orders:}

%\chaitanya{\noindent 1. Market Order: Here, the amount to be sold or bought is specified in this order type, but not the price.
%The exchange is in charge of filling the order at the lowest price possible. While market orders are frequently used to swiftly unload a "position," traders prefer alternative forms that offer them more control over the execution price.}

%\chaitanya{\noindent 2. Limit Order: A limit order defines a maximum or minimum price for the purchase or sale of a number of shares. Limit orders, unlike market orders, may not be filled if the specified price is not met. Investors can set time restrictions for order execution in some variations, beyond which the order is canceled.}

\noindent
\textit{Outgoing market data:} The CES generates a stream of real-time market data. There are multiple market participants, all located within the cloud. For each MP there is an associated Release Buffer (RB) that is controlled by the cloud-provider. Each RB receives market data directly from the CES; then it decides when the market data should be released to the corresponding MP. 

\noindent
\textit{Incoming trade orders:} Each MP generates trades based on the market data stream %(received through the RB)
and \emph{submits it} to the corresponding RB. The RB tags the incoming trade with any additional information necessary for fair ordering and forwards it to the CES. At the CES, the ordering buffer (OB) orders incoming trades based on the tagged information and forwards it to the matching engine (ME).\footnote{
To account for latency differences from MPs to the CES, the OB might need to buffer trades before forwarding them to the CES (see \S\ref{s:exp}).} 
The ME, matches buy orders against selling orders, and executes matched trade orders.% and updates the book.% \footnote{All updates to the book are published as market data.} 
%\pg{Chaitanya is this correct, are we missing something here?}

\begin{figure}[t]
\centering
    \includegraphics[width=0.8\columnwidth]{hotnets-images/FSI architecture2.pdf}
    \vspace{-2.5mm}
    \caption{\small{\bf Basic components.} RBs and OB are controlled by the cloud provider.}% \pg{Eashan see Ranveer's comment}}% \pg{Eashan can you redraw this figure in powerpoint or something.}}}
    \label{fig:basic_architecture}
    \vspace{-2.5mm}
\end{figure}

\noindent
\textbf{Notation:} 
We refer to the $x^{th}$ market data point as $x$. $(i,k)$ refers to the $k^{th}$ trade from MP$_i$. Table\ref{tab:notation} lists the notations used in this paper.


\begin{table}[h!]
\small
    \centering
    \begin{tabular}{p{0.1\columnwidth} | p{0.8\columnwidth}}
    %\hline
        \textbf{Notation} & \textbf{Definition} \\
        \hline
        $G(x)$ & Real Time at which $x$ was generated at the CES.\\
        $R_i(x)$ & Real Time at which $x$ was received at RB$_i$.\\
        $D_i(x)$ & Real Time at which $x$ was delivered by RB$_i$ to MP$_i$.\\
        $A_i(k)$ & Real Time at which $(i,k)$ was submitted by MP$_i$ to RB$_i$.\\
        $f_i(k)$ & Market data point used to generate $(i,k)$. This function is not known to anyone besides MP$_i$.\\
        $rt_i(k)$ & Response time of $(i,k)$. $rt_i(k) = A_i(k) - D_i(f_i(k))$. \\
        $O(i,k)$ & The order in which OB forwards trades to the ME. If $O(i,k) < O(j,l)$ then $(i,k)$ is ordered before $(j,l)$.
    %\hline
    \end{tabular}
    %\vspace{-2mm}
    \caption{\small{Notation.}}
    \label{tab:notation}
    \vspace{-5.5mm}
\end{table}

\if 0
\noindent
$G(x)$: Real Time at which $x$ was generated at the CES.

\noindent
$R_i(x)$: Real Time at which $x$ was received at RB$_i$.

\noindent
$D_i(x)$: Real Time at which $x$ was delivered by RB$_i$ to MP$_i$.

%\noindent
%$(i,k)$: Trade $k$ from MP$_i$.

\noindent
$A_i(k)$: Real Time at which $(i,k)$ was submitted by MP$_i$ to RB$_i$.

\noindent
$f_i(k)$: Market data point used to generate $(i,k)$. This function is not known to anyone besides MP$_i$.

\noindent
$rt_i(k)$: Response time of $(i,k)$. $rt_i(k) = A_i(k) - D_i(f_i(k))$. 

\noindent
$O(i,k)$: The order in which OB forwards trades to the ME. If $O(i,k) < O(j,l)$ then $(i,k)$ is ordered before $(j,l)$.
\fi

%\smallskip
\noindent
\textbf{Assumptions:} 

\noindent
\textit{Proximity of RB to MP:} Each RB is located sufficiently close to its MP (e.g., colocated in the same VM as the MP, \S\ref{s:disc}) and the latency between a RB and MP pair does not impact fairness.

\noindent
\textit{Communication model:} %Messages between RBs and MPs are never lost. 
%Message between a RB and the CES can get lost but it will eventually be transmitted successfully. 
Messages between a RB and the CES are delivered in-order using a reliable transport (such as TCP).
Connection disruptions can be handled using timeouts (\S\ref{s:exp}).%Latency between RBs and the CES is not bounded.
%We also assume that besides the market data stream and corresponding trades there is no other communication that can impact fairness.
We focus on trades generated directly in response to the real-time market data.
\footnote{MPs can also have access to external streams of data such as financial news streams. Compared to real-time market data, such external streams are not latency-critical and important for fairness.} %While providing fair-access to such streams is indeed possible with our framework, in the interest of space we do not consider it in this paper.}

\noindent
\textit{No failures:} We do not consider scenarios where the MPs or the CES fail. %and need to be restarted with the relevant state.
Existing solutions for replicating state machines can potentially be used to handle such failures~\cite{paxos_made_simple}. In the event of a failure, our approach will likely incur unfairness.

\subsection{Related Work}
\label{ss:related}

%CloudEx\cite{cloudex} is the closest work in this space. 
CloudEx~\cite{cloudex} leverages clock synchronization for fairness.
%to ensure that market data points are released at the same time. 
Market data $x$ is delivered simultaneously to all MPs at a pre-specified threshold ($Th$) from generation time (i.e., $D_i(x) = \max (R_i(x), G(x) + Th$). Incoming trades are simply processed in the order of submission time ($O(i,k) =A_i(k)$). An MP experiences unfairness if the latency between the CES and the MP goes beyond $Th$ and market data is delivered to it later than intended. 
%
%\attn{Increasing $Th$ can potentially help mask small latency spikes and reduce unfairness at the cost of additional latency.}
%
%\footnote{\pg{Data from production datacenters shows that network latency can increase by upto three order of magnitude in certain scenarios~\cite{google_timely}.  necessitating setting a highly of }}
%
Our approach does not require synchronized clocks. This is because, our approach only requires measuring time intervals locally at each RB. For such purposes, each RB can use its own local clock as long as the clock drift rate is small ($< 0.02\%$ in practice under a wide range of scenarios~\cite{sundial}).
%
Further, our approach can be combined with CloudEx for simultaneous delivery of market data (to the extent possible) to also provide fairness for 'one-sided' trades (see \S\ref{ss:approximate_fairness}) while also ensuring better fairness for reactive trades when latency spikes happen (\S\ref{s:exp}) or when clocks go out of sync (e.g., due to link failures ~\cite{sundial}).

\noindent
\textit{Advances in conventional networking:} There is a huge body of work~\cite{dctcp, hpcc, dcqcn, swift, hpcc, conga, bfc} (spanning congestion control, routing, kernel bypass, etc.) on reducing message transfer latencies in datacenter networks. However, none of these solutions (and none of the production datacenters) provide bounded end-to-end latency that could potentially solve the fairness problem.
%. Synchronous communication can potentially solve the fairness problem. 
In this paper, we do not attempt to change the underlying network fabric in any way. 



%\noindent 
%\chaitanya{\textit{Studies in Financial Literature:} The issue of a disconnect between economic theory and the inherent difficulties that arise when supposedly "fair" market arrangements (such as FCFS matching) are put into practice, has been well documented. The sophisticated and distributed architecture of current exchanges makes it difficult for operators to keep track of all potential sources of delays and monitor how they may effect each participant. }

%\chaitanya{Alternative market designs/order-matching strategies have been presented as solutions to account for unequal delays. For example, \cite{frequent_batch_auctions} propose a policy that interprets time as a discrete variable (rather than a continuous one) and replaces continuous auctions with "batches." This permits numerous orders to arrive at the same (separate) time, reducing the relevance of (fair or unfair) sub-millisecond submission time disparities. There is a burgeoning field developing to use mechanism design as a tool to control information transmission, as well as, to handicap participants who have an unfair advantage.}

%\noindent
%\textit{\pg{Chaitanya: related work from the financial world.}}% I am rethinking if this is needed.}}

==> hotnets/conclusions.tex <==
\section{Conclusion}
%This paper proposes a new architecture for Cloud-hosted Financial Exchanges that can provide response-time fairness, i.e. market participants that respond faster to market data are serviced first. Our system overcomes variation in link latencies and lack of accurate clock sync in the cloud through a new technique called Delivery Clocks,  which enables an ordering (DBO) with  strong fairness properties. Our scheme outperforms prior proposals that are based on enabling accurate time sync in the cloud. Although we have demonstrated the benefits of DBO in the context of a financial exchange, we note that delivery clocks will also benefit other cloud-hosted applications, such as multi-player games and ad exchanges. 
%This paper proposes a new approach for achieving response-time fairness in cloud-hosted exchanges. We introduce logical "Delivery Clocks" and show how they can be used to order trades fairly with high probability even when network latency is highly variable and clocks in the network are not synchronized. Further, while we focus on fairness for financial exchanges, our approach is general and applicable for providing fairness in many other settings such as multi-player cloud gaming and advertisement exchanges.

%This paper proposes a new approach for achieving response-time fairness in cloud-hosted financial  exchanges. We presented the concept of logical "Delivery Clocks" and showed how they can be used to order trades fairly with high probability at the presence of highly variable network latency, without requiring clock synchronization. Further, although we focussed on fairness for financial exchanges, our approach is general and suitable for providing fairness in various other settings such as multi-player cloud gaming and advertisement exchanges.

This paper proposes a new approach for achieving response-time fairness in cloud-hosted financial exchanges. We introduce the concept of logical "Delivery Clocks" and show how it can be used to order trades fairly in the presence of highly variable network latency, without requiring clock synchronization. Further, 
%although we focus on fairness for financial exchanges,
we note that our approach is general and suitable for providing fairness in other settings such as multi-player cloud gaming and advertisement exchanges.

==> hotnets/core.tex <==
%\section{How to Ensure Fairness}
%\section{Tool-kit for Fairness}
\section{Requirements for Achieving Fairness}
\label{s:core}
%\im{Perhaps title: Mechanism(s) to achieve fairness?}
%\pg{See if the notations and math is formal enough? Can we include visualizations to help (e.g., for showing what does the inter-delivery conditions mean)? Do the titles make sense? Do we need to provide more context or is it easy to follow? Most importantly do we need to provide better justification for the kind of fairness we focus on? Should we use the term RTF?}

%\noindent
%\pg{Is this start OK?}
%In this section, we will look at  properties that the delivery processes ($\cup{D_i}$) must ensure to provide fairness.

%\attn{In this section, we will establish fundamental requirements for achieving fairness. We consider different variants of fairness. Our definitions of fairness are a formal extension of the temporal fairness first introduced in~\cite{libra}. Intuitively, temporal fairness argues that trade orders from different market participants generated based on the same market data information should be ordered based on the response time of the market participants (i.e., the faster market participants orders should be submitted to the ME first). We first introduce the notion of delivery (time) based ordering. }

\attn{In this section, we will establish fundamental requirements for achieving fairness. 
We consider different variants of fairness. 
%Our definitions of fairness are a formal extension of the temporal fairness first introduced in~\cite{libra}.
%Intuitively, each variant argues that trades from different market participants generated based on the same market data information should be ordered based on the response time of the market participants (i.e., faster MP's trades should be ordered ahead of other MPs).}
%
%\eg{nit: 
At a high level, each variant argues that trades generated by different market participants based on the same market data information should be ordered based on the response time of the market participants (i.e., faster MP's trades should be ordered ahead of other MPs).}
\attn{Note that, in this section our goal is not to provide exact schemes for the delivery and ordering processes; %we do provide an exact scheme for the ordering process
rather we only aim to establish the minimum constraints on them to achieve perfect fairness.
%to facilitate those. 
We will use these constraints as guiding principles to propose concrete schemes in the next section and show that these schemes can provide fairness with a high probability. We begin by introducing delivery-time-based ordering (DBO) and showing how it can be used to improve fairness.}
\pg{Maybe present DBO case by case, starting from a single data point and two MPs responding to it.}

%We will show that the necessary conditions we derive for the delivery processes are also sufficient. In particular, we will show that if the necessary conditions for the delivery processes are met then the delivery clock time based ordering ensures fairness in each case. %\pg{Can this be made better?}

%In this section, we will look at  properties that the delivery processes ($\cup{D_i}$) must ensure to provide fairness. We will consider different variants of fairness. Our definitions of fairness are a formal extension of the temporal fairness first introduced in~\cite{libra}. Intuitively, temporal fairness argues that trade orders from different market participants generated based on the same market data information should be ordered based on the response time of the market participants (i.e., the faster market participants orders should be submitted to the ME first). We will first introduce the notion of deliver clock time based ordering. We will show that the necessary conditions we derive for the delivery processes are also sufficient. In particular, we will show that if the necessary conditions for the delivery processes are met then the delivery clock time based ordering ensures fairness in each case.

%Before we begin, we n


\smallskip
\noindent
\textit{Delivery Clock:} %The high-level idea here is that 
\attn{%Competing MPs don't make trade decisions in isolation rather they place trades directly in response to same market data stream. 
Competing MPs make trade decisions directly in response to the same market data stream.}
%For trade decisions,} 
Events corresponding to the delivery of the same market data point to different MPs, thus, relate to the same conceptual event. %To capture this relationship, e
Each RB maintains a separate delivery clock to track these conceptual events. Delivery clock is represented by a lexicographical tuple and it increases monotonically with time. Formally, delivery clock at RB$_i$ at time $t$ is given by,
\begin{align}
    DC_i(t) = \langle x_l(t), t-D_i(x_l(t))\rangle.
\end{align}
where $x_l(t)$ is the latest data point that was delivered to MP$_i$ (i.e., $D_i(x_l(t)) \leq t < D_i(x_l(t)+1)$). Interval, $t-D_i(x_l(t))$, corresponds to the time that has elapsed since the latest delivery.\footnote{$t-D_i(x_l(t))$ can be computed based on the local clock of RB$_i$.}% as long as the clock drift rate is small.}.
This tuple tracks the progress of market data delivery to the corresponding MP. 

\begin{figure}[t]
\centering
    \includegraphics[trim={0 0 0 2mm},clip,width=0.9\columnwidth]{hotnets-images/time series visualization (3).pdf}
    \vspace{-3mm}
    \caption{\small{{\bf DBO can help correct for late delivery of data.} Delivery of market data to MP$_i$ is lagging behind MP$_j$. There are two trades $(i,k)$ and $(j,l)$ generated in response to the same market data $x$. $(j,l)$ was submitted before $(i,k)$ but
    %, i.e., $A_j(l) < A_i(k)$. 
    response time of $(i,k)$ is less than $(j,l)$.
    %, i.e., $rt_i(k) < rt_j(l)$. 
    With DBO, $O(i,k) (= \langle x, rt_i(k)\rangle) < O(j,l) (= \langle x, rt_j(l)\rangle)$ and trade $(i,k)$ is correctly ordered ahead of $(j,l)$. Ordering based on the submission time leads to incorrect ordering.}}
    \label{fig:dbo_correction}
    \vspace{-4mm}
\end{figure}
%\pg{Eashan see if you can redraw this for clarity.}} %\eg{$A_j(l)<A_i(k)$ and $rt_i(k)<rt_j(l)$. Even though trade order from $\text{RB}_j$ is submitted to the exchange network before $\text{RB}_i$, according to DBO, $\text{RB}_i$'s request should be executed first due to its lower response time i.e. $O(i,k) (= <x, rt_i(k)>) < O(j,l) (= <x, rt_j(l)>)$.}}\pg{Eashan redraw this.}}

\vspace{-1mm}
\begin{definition}
DBO satisfies the following condition,
\begin{align}
O(i,k) = DC_i(A_i(k)).
\end{align}
\vspace{-6mm}
\end{definition}

\attn{With DBO, trades are ordered based on the RB \emph{delivery clock time at trade submission}.\footnote{\attn{For DBO, each RB can tag this delivery clock time in trades before forwarding them to the CES.}} In other words, DBO is ordering trades from MPs relative to when they received the market data. }
Intuitively, DBO can be thought of as a post hoc way of correcting for time differences in delivery of market data to MPs. % (due to, for example,  high latency from the CES to a particular MP). 
For example, if market data delivery to a particular MP lags behind other MPs (e.g., due to a latency spike), then its delivery clock also lags behind. Compared to ordering trades based on the submission time, with DBO, trades from this MP receive a boost in ordering that can correct for the late delivery (example in \Fig{dbo_correction}). \pg{Another way of thinking about DBO is that (loosely speaking) it creates the perception that each MP has the same RTT to the CES. Roughly speaking, incoming trades from MPs are delayed in inverse proportion to the delay experienced in market data delivery (see Handling latency variation on the reverse path in \S\ref{s:exp}).}


%\Fig{dbo_correction} illustrates this in a simple scenario. 
% \eg{With DBO, trades are ordered based on the delivery clock time at trade submission to the corresponding RB. In other words, DBO is ordering trades from MPs relative to when they received the market data. For example, if market data delivery to a particular MP lags behind other MPs (say due to a latency spike), then its delivery clock compared to other MPs also lags behind. Compared to ordering trades based on the real time at submission, with DBO, trades from this MP receive a boost in ordering that can correct for the late delivery (example in \Fig{dbo_correction}).}

%\pg{Eashan a figure to illustrate this would be super useful.}
%
%(due to, for example,  high latency from the CES to a particular MP).
%

DBO alone is capable of partially correcting differences in market data delivery across MPs. Perfect correction, would require measuring the response time of a trade. The challenge, however, is that a trade could have been generated in response to any of the market data points delivered to the MP (and not just the latest data point $x_l$). The RB/OB cannot trust the MP to truthfully offer this information. We show that we can alleviate this issue by enforcing certain restrictions on how the delivery clocks advance across RBs (i.e., restrictions on the pace of market data delivery to the MPs). 

We will now derive the minimum requirements on the delivery processes for achieving fairness for arbitrary trade orders for \emph{any} ordering process.\footnote{We assume that $f_i$ is not known to the ordering process.} We will also show that if these delivery requirements are met,  DBO ensures perfect ordering for fairness. 

\subsection{Strong Fairness}
\label{ss:strong_fairness}
%\pg{Eashan verify if the theorems and are corollaries are indeed correct. Pay special attention to whether it should be $<$ ot $\leq$.}

\begin{definition}
An ordering process $O$ is strongly fair if it satisfies the following conditions,
\begin{align*}
    C1: &\text{ If } A_i(k) < A_i(l), \text{ then, } O(i,k) < O(i,l).\nonumber\\
    C2: &\text{ If } f_i(k) = f_j(l) \land rt_i(k) < rt_j(l), \text{ then, }
    O(i,k) < O(j,l).
\end{align*}
\label{def:strong}
\vspace{-5mm}
\end{definition}

%Condition $C1$ states that a MP is always better-off submitting the trade order as early as possible and waiting to submit trade orders does not offer any advantage.
Condition $C1$ states that a MP is always better-off submitting the trade order as early as possible. $C2$ states that trade orders generated based on the same market data point should be ordered based on the response time of the MPs.% (i.e., faster MP's trades should be ordered ahead).}
%$C2$ states that trade orders generated based on the same market data point should be ordered based on the response time of the MPs.} %.%forwarded to the ME first). 


\begin{theorem}
The \textit{necessary} and \textit{sufficient} conditions on the delivery processes for strongly fair ordering are given by,
\begin{align*}
    D_i(x+1) - D_i(x) &= D_j(x+1) - D_j(x), & \forall i,j,x.
\end{align*}
\label{thm:1}
\vspace{-6mm}
\end{theorem}

The theorem states that for strong fairness the inter-delivery times should be the same across all  MPs. In other words, the delivery clocks at all RBs (at any given delivery clock time) must advance at the same rate.

% eg{The theorem states that, for strong fairness, the intervals between consecutive market data deliveries -- inter-delivery times -- should be the same across all MPs. In other words, the delivery clocks at all RBs (at any given delivery clock time) must advance at the same rate.}

\begin{proof}
\textit{Necessary:} To prove that the above condition is necessary we will show that if this condition is not met then no ordering process exists which is strongly fair for arbitrary trade orders. %\attn{We will constuct a tra}%already said this %
%The reason for this is that the OB does not know the response time of trade orders ($\sum f_i$ is unknown). 

\begin{figure}[t]
\centering
    \includegraphics[trim={0 0 0 1mm},clip,width=0.8\columnwidth]{hotnets-images/delivery times.pdf}
    \vspace{-3mm}
    \caption{{\small{\bf Proof of Theorem 1.}}}% \pg{Eashan include as an arrow for progress of time.}}
    \label{fig:proof}
    \vspace{-5mm}
\end{figure}

Consider the following scenario (\Fig{proof}) where the above condition is not met. Let $D_i(x+1) - D_i(x) = c1$, $D_j(x+1) - D_j(x) = c2$. Without loss of generality we assume $c1<c2$. Consider hypothetical trades $(i,k)$ and $(j,l)$ s.t. $A_i(k) = D_i(x+1) + c3$ and $A_j(l) = D_j(x+1) + c4$. Further, we can pick $A_i(k)$ and $A_j(l)$ s.t. $c3>c4$ and $c1+c3<c2+c4$. Now we consider two scenarios for how these trades were generated. These two scenarios are indistinguishable at the OB.
%Consider a hypothetical trade order $k$ (from MP$_i$) and $l$ (from MP$_j$) s.t. $A_i(k) = D_i(x+1) + c3$ and $A_j(l) = D_j(x+1) + c4$. Further, we can pick $A_i(k)$ and $A_j(l)$ s.t. $c3>c4$ and $c1+c3<c2+c4$. Now we consider two scenarios for how these trades were generated. These two scenarios are indistinguishable at the OB.

\noindent
\text{Case 1:} $f_i(k) = f_j(l) = x+1$. Here,
\begin{align}
rt_i(k) = c3, rt_j(l) = c4.
\end{align}
Since $c3>c4$, a strongly fair ordering (condition $C2$) must satisfy,
%\begin{align}
$O(i,k) > O(j,l)$.
%\label{eq:theorem_1:necessary:case1}
%\end{align}

\noindent
\text{Case 2:} $f_i(k) = f_j(l) = x$. Here,
\begin{align}
rt_i(k) = c1+c3, rt_j(l) = c2+c4.
\end{align}
In this case, since $c1+c3<c2+c4$, a strongly fair ordering must instead satisfy the opposite, $O(i,k) < O(j,l)$. A contradiction! \attn{Thus, no ordering process can be strongly fair in both these scenarios.}
%\label{eq:theorem_2:necessary:case1}
%\end{align}


\smallskip
\noindent
\textit{Sufficient:} We will now show that if the inter-delivery times are same across MPs, then a strongly fair ordering exists. 

Assuming same inter-delivery times, DBO trivially satisfies $C1$. DBO also satisfies $C2$, i.e.,  if $f_i(k) = f_j(l) \land rt_i(k) < rt_j(l)$, then,
\begin{align}
    DC_i(A_i(k)) < DC_j(A_j(l)). 
\end{align}
Intuitively, this is because market data $f_i(k) (= f_j(l))$ is delivered to each MP at the same delivery clock time (by definition). Further, delivery clocks advance at the same rate across all MPs. When measured from the delivery of $f_i(k) (= f_j(l))$, delivery clock of RB$_j$ in duration $rt_j(l)$ will advance more than delivery clock of RB$_i$ in duration $rt_i(k)$.
Therefore, DBO is strongly fair.\footnote{\attn{Note that, DBO is not the only ordering process that can achieve strong fairness. Other ordering processes that also order trades from MPs based on when they received the market data can also achieve strong fairness.}} 
\end{proof}

\if 0
Assuming same inter-delivery times, DBO trivially satisfies $C1$. DBO also satisfies $C2$. If $f_i(k) = f_j(l) \land rt_i(k) < rt_j(l)$, then,
\begin{align}
    DC_i(A_i(k)) < DC_j(A_j(l)). 
\end{align}
% \eg{
% \begin{align}
%     DC_i(A_i(k)) = \langle x^i_l, rt_i(k)+(D_i(f_i(k))-D_i(x^i_l)) \rangle < DC_j(A_j(l)) = \langle x^j_l, rt_j(l)+(D_j(f_j(l))-D_j(x^j_l)) \rangle. 
% \end{align}}
Intuitively, DBO satisfies $C2$ because market data $f_i(k) (= f_j(l))$ is delivered to all the MPs at the same delivery clock time (by definition). Because delivery clocks advance at the same rate across all MPs, (measured from the delivery of $f_i(k)$) delivery clock of RB$_j$ in duration $rt_j(l)$ will have advanced more than delivery clock of RB$_i$ in duration $rt_i(k)$.
Therefore, DBO is strongly fair. 
%\end{proof}
\fi

\noindent
\textit{On impossibility of strong fairness:} It is possible to show that if communication latency is not bounded then RBs cannot %coordinate \im{co-ordinate implies talking to each other; another word perhaps?} to
achieve the same inter-delivery times always. %(if the market data stream is not known in advance \im{I don't understand this text in the parenthesis}). 
In the interest of space we skip this proof. The high-level idea is that if two RBs can achieve the same inter-delivery times then they can also agree to execute some task (not known at the start) simultaneously. 
%From earlier work on the folklore two-generals-problem~\cite{two_generals} it is well known that is impossible if the communication latency is not bounded.\eg{some rephrasing required: 
From earlier work on the folklore two-generals-problem~\cite{two_generals}, it is well known that such simultaneous execution is impossible if the communication latency is not bounded. While it might not be possible to achieve the same inter-delivery times all the time, we can achieve it with high probability at the cost of some additional latency at the RB~\cite{cloudex}.% \pg{check if the citation is correct, maybe a better one exists.}

Next, we consider two weaker variants of fairness. We give the necessary and sufficient conditions for the delivery processes in each case. The proofs in each case are similar to that of Theorem~\ref{thm:1}. We can construct a counter example to show that the conditions are necessary. For sufficiency, we can show that if the conditions are met then DBO satisfies the fairness properties. Depending on the needs of the application one can also consider alternate definitions of fairness, derive the desired properties and construct schemes that try to ensure these properties for fairness.

\subsection{Limited Fairness}
\label{ss:limited_fairness}
\vspace{-1mm}
\begin{definition}
An ordering process $O$ ensures limited fairness if it satisfies $C1$ and the following condition,
\begin{align*}
    C3: \text{If } f_i(k) &= f_j(l) \land rt_i(k) < rt_j(l) \land rt_i(k) < \delta, \text{ then},\nonumber\\
    O(i,k) &< O(j,l).
\end{align*}
\vspace{-5mm}
\end{definition}
%\im{that should be $rt_i(k) < rt_j(l)$ correct? If yes, please fix}
where $\delta$ is a positive constant.

Intuitively, $C3$ states that if the response time of a MP is bounded, then its trades will ordered ahead of corresponding trades from other MPs as long as it is faster than other MPs.
This definition is most relevant in the high frequency trading world where the response time is in the order of a few microseconds. 
%(\pg{Chaitanya can we motivate this definition better}). %\eg{can we say, "The reason for unfairness is the unequal transmission delays in the network, the variance of which in a high performance network is of the order of $100\mu s$. Following this, we may be only concerned with fairness for trades within an appropriate $\delta$ so as to provide all fast MPs a fair platform."}\pg{I dont understand your comment}

\vspace{-1mm}
\begin{corollary}
The \textit{necessary} and \textit{sufficient} conditions on the delivery processes for limited fairness are given by,
\begin{align*}
    \text{If }  D_i(x+1) - D_i(x) &< \delta, \text{ then},\nonumber\\
    D_j(x+1) - D_j(x) &= D_i(x+1) - D_i(x), & \forall j.
\end{align*}
\label{cor:1}
\vspace{-5mm}
\end{corollary}


%\im{leeway or headroom instead of slack? not sure}
Compared to strong fairness, the above condition offers some leeway for how the delivery clocks can advance. \attn{If for a certain MP, the inter-delivery time for two consecutive data points is greater than equal to $\delta$, then for any other MP, the inter-delivery for these points can differ as long as it is greater then $\delta$.}
%In particular, for certain market data points the inter-delivery times across MPs need not be the same as long as the inter-delivery time for such points at each MP $\geq \delta$. 
This leeway is useful for dealing with sudden latency spikes. In the next section, we will consider a simple scheme for the delivery processes that meets the above condition at all times %(for any value of $\delta$)
regardless of the fluctuations in latency.

%I like what you have, let me think more.
%Compared to strong fairness, the above condition offers some leeway for how the delivery clocks can advance. For example, in case of sudden latency spikes, as long as all MPs maintain inter-delivery times larger than $\delta$, the MPs can pace data delivery accordingly so as to handle the unexpected delays \sout{while ensuring the fairness property}. In the next section, we will consider a simple scheme for the delivery processes that meets the above \sout{fairness} condition at all times regardless of the fluctuations in latency.

\subsection{Approximate Fairness}
\label{ss:approximate_fairness}
\begin{definition}
An ordering process $O$ is approximately fair if it satisfies $C1$ and the following condition,
\begin{align*}
    C4: \text{If } f_i(k) &= f_j(l) \land rt_i(k) \cdot (1+\epsilon)< rt_j(l), \text{ then},\nonumber\\
    O(i,k) &< O(j,l),
\end{align*}
\vspace{-6mm}
\end{definition}
where $\epsilon$ is a positive constant.

Intuitively, $C4$ states that as long as a MP is faster than other MPs by a certain margin, it's trades will be ordered ahead.%submitted to the ME earlier.

\vspace{-1mm}
\begin{corollary}
The \textit{necessary} and \textit{sufficient} conditions on the delivery processes for approximately fair ordering are given by,
\begin{align*}
    D_i(x+1) - D_i(x) &\leq (D_j(x+1) - D_j(x)) \cdot (1 +\epsilon), & \forall i,j,x.
\end{align*}
\label{cor:2}
\vspace{-6mm}
\end{corollary}

Compared to strong fairness, the above condition also offers some leeway for inter-delivery times to differ. This leeway can be useful for masking fluctuations in latency (\S\ref{s:exp}). %\pg{Include a note on how this relates to clock drift rate?}

\smallskip
\noindent
\textit{Do we need clock-sync?} For fairness, RBs only need to ensure the specified constraints for inter-delivery times in each case. Ensuring these contraints does not require clock synchronization across RBs. A RB can use its own local clock for maintaining inter-delivery times as long as the clock drift rates are small.
%\footnote{It is possible to analyze the impact of high clock drift rates on fairness. Due to space constraints, we exclude it.} 
With perfect clock synchronization, RBs can additionally ensure that market data is released at the same time when not experiencing extreme fluctuations in network latencies. 
%Furthermore, with clock synchronization among RBs, DBO could additionally ensure fairness for `one-sided' trades (generated independently of the current market data -- e.g, limit orders) that ideally should be ordered based on the time when they were submitted.
Furthermore, simultaneous delivery of market data also syncs the delivery clocks at RBs. In such cases, DBO additionally provides fine-grained fairness (similar to that of CloudEx) for `one-sided' trades (generated independently of the current market data) % -- e.g, limit orders)
that ideally should be ordered based on the time when they were submitted.
%\pg{chaitanya please check this part about one sided orders, example of one side orders, how important is fairness for such one sided trades, not sure if this is needed}%\pg{does this make sense? should we say fairness for one-sided orders is less important or the time scales are less relavent (similar to our argument for trades based on non-real time data).}

%\pg{Ensuring these inter-delivery constraints does not require access to clock sync }

==> hotnets/discussion.tex <==
\section{Discussion}
\label{s:disc}
%We discuss few additional challenges in moving financial exchanges to the cloud.

%\subsection{Implementation of a delivery clock system}

\subsection{DBO Cloud Architecture}
%\pg{Ilias, I wonder is this should be 5.2 instead}\pg{maybe cut short}

In a typical on-premise deployment, the CES servers and physical network are part of the trusted infrastructure of the exchange: the exchange operators have exclusive access to the physical machines, and network cables. On the other end, the MPs own the physical servers that connect to the exchange network. Migrating such components to the public cloud seems intuitive: CES servers and MPs could correspond to virtual machines owned by the different parties.

Compared to on-premise deployments one important differentiation is that our solution requires the use of Release Buffer components for correctness, hence those need to be part of the trusted infrastructure (i.e., the MPs should have no control over the RBs). As we have discussed, the RBs should be close enough to the MPs, so that the latency between them does not impact fairness. The Release Buffer components need to {\it pace} the delivery of data to MPs. The cloud operator could provide the facilities required for the RB functionality. We believe that such functionality, could potentially be embedded in many places such as the hypervisor of cloud nodes that host MPs, or better the programmable NIC of such cloud hosts (most operators already have their own programmable smartNICs~\cite{accelnet} deployed). There are several challenges that need to be considered such as performance isolation, but the cloud operator already has fine-grained control over the cloud hardware/software stack and can address this problem easily. %One other option worth exploring for the release buffer functionality, would be the use of programmable Top-of-Rack switches~\cite{tofino}.



%\subsection{Multi-machine, Multi-cloud, Multi-exchange}
%\label{ss:multi}
\subsection{Enabling a MP to use many machines}
\label{ss:multi_machine}
%\pg{Chaitanya: citation for front running attack.}
So far, we have assumed that each MP is a single machine (or a virtual machine) sitting in the cloud. However, a single machine might not be enough and a MP might want to use multiple ``helper'' machines for computation. These helper machines can be located either in the cloud or outside the cloud (e.g., a MP might want to run its own on-prem datacenter). The ``front-end'' machine of the MP (that is receiving the real-time market data from the RB) should be able to communicate with these helper machines. 

Allowing such communication naively can lead to ``front-running'' attacks. In principle, a MP (whose delivery clock is lagging behind) might be able to receive real-time market data from another MP earlier than receiving it from the CES. Since, trades are ordered based on the delivery clock, earlier access to market data gives such a MP an unfair advantage over other MPs. 
It is possible to ensure that no MP gets early access to market data %(at the cost of introducing latency in messages from the front-end to helpers outside the cloud)
and thwart such front-running attacks. Here, we give a rough sketch of the solution. 
%
%\pg{Which of two alternatives is better?}
%
There are two simple constraints. \begin{enumerate*}[label=(\arabic*)]\item Only the front-end of a MP is allowed to submit the trade orders. 
\item Any data (excluding the trade orders) from the front-end to any other machine is buffered at the corresponding RB until the RB is sure that the delivery clocks at all other RBs have advanced beyond its delivery clock when it received this data.\end{enumerate*} A simple way to achieve this is for each RB to send other RBs periodic beacons communicating the status of its delivery clock. This way each RB can maintain a lower bound on the delivery clocks at other RBs. There are other ways to thwart front-running that impose weaker restrictions on communication or are easier to implement. We chose to present this one for its simplicity.

% \eg{There are two simple constraints. \begin{enumerate*}[label=(\arabic*)]\item Only the front-end of a MP is allowed to submit the trade orders. \item Any data (excluding the trade orders) from the front-end is buffered by the cloud network to make sure that the delivery clocks at all other RBs have advanced beyond the delivery clock time when this data transmission was initiated.\end{enumerate*} A simple way to ensure this is to transmit all outgoing data through the RB and for each RB to send periodic beacons communicating the status of it's delivery clock. This way each RB can maintain a lower bound on the delivery clocks at other RBs. Note that there are other ways to thwart front-running that impose weaker restrictions on communication or are easier to implement. We chose to present this one for it's simplicity.}

\if 0
\pg{There are three simple constraints. (1) Only the front-end of a MP is allowed to submit the trade orders. (2) A helper within the cloud is only allowed to talk to it's MP's front-end and helpers in the cloud. 
%Most cloud-providers already employ proxies that can be used to enforce this restriction.  
(3) Any data (excluding the trade orders) from the front-end to other machines (excluding the MP's helpers in the cloud) is buffered at the corresponding RB until the RB is sure that the delivery clocks at all other RBs have advanced beyond its delivery clock when the it received this data. A simple way to achieve this is for each RB to send other RBs periodic beacons communicating the status of it's delivery clock. This way each RB can maintain a lower bound on the delivery clocks at other RBs.}
\fi


\if 0
Only the front-end of a MP is allowed to submit trade orders. %\pg{Add a note on why this additional latency is not bad?Chaitanya can we say that typically a MP's fast computations can fit within a VM or something?}

\noindent
\textit{Helpers in the cloud:} Such a helper is only allowed to talk to it's MP's front-end and helpers in the cloud. Most cloud-providers already employ proxies that can be used to enforce this restriction.

\noindent
\textit{Helpers outside the cloud:} Such a helper can talk to any machine outside the cloud (including helpers of other MPs). But, it is only allowed to talk to the corresponding front-end in the cloud. Any data from the front-end to outside the cloud is buffered at the corresponding RB until the RB is sure that the delivery clocks at all other RBs have advanced beyond its delivery clock when the it received this data.%\footnote{To avoid buffer overruns at the RB, the outgoing data can also be buffered at other points in the network at the cost of some additional latency.} 
A simple way to achieve this is for each RB to send other RBs periodic beacons communicating the status of its delivery clock. This way each RB can maintain a lower bound on the delivery clocks at other RBs. %The above mechanism ensures that a MP cannot have earlier access to market data from another MP.

\fi






\subsection{Enabling a MP to use a different cloud-provider}
A MP might prefer a different cloud-provider (for its front-end and helpers) than the one the financial exchange is located in. 
%or offer lower latency between the front-end and helpers that could help the MP to make trade decisions faster. 
Achieving fairness in such scenarios requires participating cloud-providers to agree on a common implementation of the RB and being truthful in tagging trades for DBO. Further, to keep end-to-end latency low, cloud-providers will likely need to enter peering agreements~\cite{sky}. %to keep the cross-cloud latency in check. 
While there are many challenges in realizing this vision, we believe our approach for fairness will prove to be even more useful here.\footnote{Achieving tight clock synchronization at RBs across cloud providers will likely be harder~\cite{huygens} and latency across clouds is likely more unpredictable.}



\subsection{Fairness with multiple exchanges}
\attn{
%To our knowledge, 
Existing financial exchanges %(and proposed solutions) 
do not optimize for ensuring fair-access to market data streams from other financial exchanges. Currently, competing financial exchanges are not colocated. MPs can go to great lengths to reduce latency for market data streams from financial exchanges that they are not colocated with~\cite{frequent_batch_auctions}.
%\footnote{\attn{For example, Spread Networks spent 300 million dollars for a private fiber optic cable to help HFT firms in New York connect to financial exchanges in Chicago and vice-versa~\cite{frequent_batch_auctions}.}}
In future, if multiple financial exchanges move to the cloud, participating cloud providers can take up the task of ensuring fairness across data streams from all such exchanges. A potential way to do this is to stitch together all such data streams into a single stream using a common serialization point. %\footnote{\attn{Creating such a single stream will likely require competing financial exchanges to agree on a fair ordering of their data in this stream.}} 
Our approach can then be used to order trades fairly based on the delivery time of the data in this super stream. Such an ecosystem offers a lot of flexibility and can enable both MPs and financial exchanges to move across cloud regions and cloud providers to optimize cost and performance.}




\if 0
\subsection{Beyond Fairness}

While the focus of this article has been on fair market access, market regulations also have additional implications.

1) Market Transparency and Coordination: Because traders trade and hedge across numerous markets, there are significant interdependencies between them. Markets must be transparent and coordinated in order to achieve efficiency and the best pricing. The National Best Bid or Offer (NBBO) rule established this obligation (Reg NMS, 1972 and 2005).

2) Market Surveillance: Because markets are so important to the economy's general stability, exchanges are essential to avoid market manipulation and fraud. This is accomplished through the use of audit trails, surveillance, and disciplinary measures. To do so, the exchanges can use cloud hosting to have access to machine learning techniques and infrastructure.

3) Market Stability and Systemic Risks: Exchanges must also have enough capacity to deal with big trading volumes and spikes.

Low latency and real-time data access are frequently required by these needs. However, cloud virtualization and sharing overheads prevent this. The "Lift and Shift" method is ineffective.


Another difficulty is replicating the "determinism" of an on-premise solution. Exchanges must, in particular, ensure that transactions are processed in a logical order based on entry time and priority. This is complicated by the cloud's inherent jitter. Kernel by-passes that give access to low-level network card controls, as well as intelligent workload placement such as avoiding workload sprawl, co-locating similar workloads in close proximity, and isolating nodes when latency-sensitive workloads are operating, can help address these issues. Each of these tasks necessitates the development of new algorithms.
\fi


%\subsection{Requirements beyond fairness}
%\pg{Chaitanya, since we are running over if we can wrap it within half a column it would be great.}



==> hotnets/introduction_new.tex <==
\section{Introduction}
\label{s:introduction}

Cloud providers are continuously improving their datacenters to provide better computing, networking and storage resources to end customers. These innovations have helped many industries to forego the cumbersome task of building and maintaining their own on-premise data centers and move to the cloud. Despite all the investment and innovation from cloud providers, however, cloud environments today are still not well suited for many industries.

%Most of the major financial exchanges (such as NASDAQ, CME, NYSE) run their Central Exchange Server (CES) in  on-premise data centers. At a high level, the CES generates market data and distributes it to various market participants (MPs) in real time. Fairness with regards to the market data stream, would constitute simultaneous data delivery to all market participants. In modern financial exchanges such fairness is not a commodity but rather comes at a premium: MPs that are interested in earliest possible delivery of the market data, are paying high fees to collocate their servers in the financial exchanges' data centers as close as possible to the exchange's Matching Engine (ME). Such MPs (commonly known as high-frequency traders), rapidly react\footnote{High frequency traders are very aggressive in reducing latency: they often use programmable smartNICs to shave off just ns of latency on their end to gain competitive advantage.} to new market data generating a high volume of transactions: their profit is highly dependent on winning the `race for speed', aiming to submit their trade transactions before other competing MPs. For the rest of the MPs there is no guarantee with regards to market data delivery (data are streamed over variable-latency private or public WAN links). \attn{Fairness with regards to trade orders processing, would constitute processing them sorted based on their response time since the delivery of the actual market data. } A property that would be sufficient to achieve both of the aforementioned types of fairness is ensuring provable equal bi-directional latency between the CES and the colocated MPs. Such property immediately guarantees simultaneous delivery of market data to the colocated MPs, while a simple First Come, First Served (FCFS) for orders processing would be sufficient to ensure fairness with respect to response time. The financial exchanges often go to great lengths in achieving equal bi-directional latency between the CES and the colocated MPs: It is not uncommon, for example, for exchanges such as NASDAQ to use equal-length cables for all colocated MPs to achieve provably equal bidirectional latency.

\iffalse
Most of the major financial exchanges (such as NASDAQ, CME, NYSE) run their Central Exchange Server (CES) in  on-premise data centers. At a high level, the CES generates market data and distributes it to various market participants (MPs) in real time. Fairness with regards to the market data stream, would constitute simultaneous data delivery to all market participants. In modern financial exchanges such fairness is not a commodity but rather comes at a premium: MPs that are interested in earliest possible delivery of the market data, are paying high fees to collocate their servers in the financial exchanges' data centers as close as possible to the exchange's Matching Engine (ME). Such MPs (commonly known as high-frequency traders), rapidly react\footnote{High frequency traders are very aggressive in reducing latency: they often use programmable smartNICs to shave off just ns of latency on their end to gain competitive advantage.} to new market data generating a high volume of transactions: their profit is highly dependent on winning the `race for speed', aiming to submit their trade transactions before other competing MPs. For the rest of the MPs there is no guarantee with regards to market data delivery (data are streamed over variable-latency private or public WAN links). \attn{Fairness with regards to trade orders processing, would constitute processing them sorted based on the time they were generated.} A property that would be sufficient to achieve both of the aforementioned types of fairness is ensuring provable equal bi-directional latency between the CES and the colocated MPs. Such property immediately guarantees simultaneous delivery of market data to the colocated MPs, while a simple First Come, First Served (FCFS) for orders processing would be sufficient to ensure fairness with respect to response time. The financial exchanges often go to great lengths in achieving equal bi-directional latency between the CES and the colocated MPs: It is not uncommon, for example, for exchanges such as NASDAQ to use equal-length cables for all colocated MPs to achieve provably equal bidirectional latency.
\fi

%Most of the 
Major financial exchanges such as NASDAQ, CME, and NYSE run their Central Exchange Server (CES) in on-premise data centers. At a high level, the CES generates market data and distributes it to various market participants (MPs) in real time. Certain MPs (commonly known as high-frequency traders), rapidly \emph{react} to new market data issuing a high volume of transactions: their profit is highly dependent on winning the `race for speed', aiming to submit their trade orders before other competitors.\footnote{High frequency traders are very aggressive in reducing latency: they often use programmable smartNICs to shave off just $\mu\,s$ of latency on their end to gain competitive advantage.}
To accommodate fair competition based on speed of trading, modern financial exchanges offer simultaneous delivery of market data to the interested MPs, as well as ordered processing of the trade transactions based on their submission time \attn{(measured at the MP)}. Such fairness is only  provided to a fraction of the MPs, and comes at a premium cost: financial exchanges offer colocation services for MPs' servers at the same datacenter as the exchange's CES, where they are able to provably guarantee equal bidirectional latency from the CES to all colocated MPs. Exchanges go to a great extent to ensure fairness for their colocated MP customers; it is not uncommon, for example, to use layer-1 fan-out switches for market data stream replication and equal-length cables to all colocated MPs.
%for provably equal bi-directional latency. 
For the rest of the MPs -- who either do not profit from such trading strategies or cannot afford the colocation services -- fairness of such kind is not available. Such MPs typically receive the market data stream and submit orders over variable-latency private or shared WAN links, or through intermediate brokers.

% \eg{Most of the major financial exchanges such as NASDAQ, CME, and NYSE run their Central Exchange Server (CES) in on-premise data centers. At a high level, the CES generates market data and distributes it to various market participants (MPs) in real time. Certain MPs (commonly known as high-frequency traders), rapidly \emph{react} to new market data issuing a high volume of transactions: their profit is highly dependent on winning the `race for speed', aiming to submit their trade orders before other competitors\footnote{High frequency traders are very aggressive in reducing latency: they often use programmable smartNICs to shave off just $\mu\,s$ of latency on their end to gain competitive advantage.}.
% To accommodate fair competition based on speed of trading, modern financial exchanges offer simultaneous delivery of market data to the interested MPs to a fraction of the MPs at a premium cost: financial exchanges offer colocation services for MPs' servers at the same datacenter as the exchange's CES, where they are able to provably guarantee equal bidirectional latency from the CES to all colocated MPs. Exchanges go to a great extent to ensure fairness for their colocated MP customers; it is not uncommon, for example, to use layer-1 fan-out switches for market data stream replication and equal-length cables to all colocated MPs. For the rest of the MPs -- who either do not follow such trading strategies or cannot afford the colocation services -- fairness of such kind is not available. Such MPs typically receive the market data stream and submit orders over variable-latency private or shared WAN links, or through intermediate brokers.}

Moving the CES to the cloud presents a huge business opportunity for major cloud providers such as Amazon, Google, and Microsoft~\cite{nasdaq_cme_an, nasdaq_aws}. Financial exchanges also have a strong incentive to move their business to the cloud: they could rapidly increase market access to more participants, and also benefit from modern cloud's elastic resource scaling. To achieve smooth migration to the cloud, however, all of modern exchanges' services need to be accommodated, including fairness on speed trading which presents unique challenges. In particular, ensuring fairness by providing deterministic equal latency to the MPs similar to the on-premise datacenters, would be quite challenging in the cloud. Cloud datacenters have originally been designed for a heterogeneous, multi-tenant environment, aiming to accommodate diverse workloads. Even if the MPs are located within the same cloud region as the CES, it is hard to guarantee that the latency between CES and various MPs will be the same. Copper and fiber optics cables are not necessarily of equal length, network traffic is not evenly balanced among the different paths, multiple vendors' network elements have different performance characteristics, network oversubscription is still common in datacenters, and network quality of service mechanisms for concurrent workloads are only best effort.


Over the recent years, this problem has received some attention from both the financial and computer science research communities.
%to counter the asynchronous communication constraint. 
CloudEx~\cite{cloudex} proposes using high-precision clock synchronization to ensure that the market data is released %(at vantage points located very close to the MPs)
to MPs simultaneously along with ordering trades based on the submission time. In the event of latency spikes beyond a certain threshold, however, CloudEx incurs unfairness. Unfortunately, production datacenters do not guarantee bounded latency. Latency spikes (up to a few orders of magnitude increase than average) are quite frequent due to a multitude reasons such as congestion~\cite{google_timely}, and link failures~\cite{conga}. \pg{Maybe make the point that no algorithm can ensure simultaneous delivery of data with unbounded latency (two generals problem).}
Libra~\cite{libra} orders incoming trade requests based on their contents %(e.g., the selling price offered by the MP for an instrument). 
while Budish et al.~\cite{frequent_batch_auctions} propose aggregating real-time market data and delivering it in batches to the MPs along with aggregating incoming trades corresponding to a batch. These approaches, however, impose significant restrictions as they require changes to how trades are processed at the CES~\cite{cloudex}.% and can introduce inefficiencies (\S\ref{s:exp}).}


In this paper, we set out to tackle the problem of providing fairness for financial exchange systems that operate in modern cloud datacenters. We observe that provably equal latency between CES and MPs is a useful property that helps ensuring equal opportunity for market participants, but it is both hard to achieve and not strictly essential for the purpose. Instead, for our solution we adopt a radically different approach: we choose to relax any assumptions for tight clock synchronization among cloud nodes or predictable bounded latency in datacenter networks. Further, our approach is general since it does not require any changes to the core central exchange algorithms. 
Our key premise is that, simultaneous delivery of market data is only essential for \emph{reactive} trades that are generated directly and quickly in response to specific real-time market data points~\cite{libra}. For all other trades, minor differences in delivery times are not critical.\footnote{Our approach can leverage clock synchronization to additionally provide fine-grained fairness for such trades (\S\ref{s:background}).}  For such reactive trades, we do not need to ensure simultaneous delivery of market data. We can alternatively achieve fairness by enforcing {\it ordering} on incoming trade requests based on the duration it took for each participant to react, \attn{i.e, time taken to submit a trade since the reception of some particular market data (response time).}
%(i.e, submit a trade) upon the reception of some particular market data (response time).%\pg{is this our insight?}


%\sout{With such an approach, we shift the problem from the datacenter network to the cloud end hosts, where operators have more flexibility and tighter control. \pg{Doesn't CloudEx also do this?}}
% \pg{say ensuring equal or even bounded latency might be hard and even not possible. Maybe we should say that our solution is capable of providing some/better fairness when clocks go out of sync or latency spike happens.}

%\pg{Ilias should we move the next two paragraphs to the related work section? I am not sure, I rewrote them a little.}
%\attn{The challenge in ordering trades this way is that it is hard to measure response times since the cloud-provider does not know how the MP generated a specific trade (i.e., which data triggered the trade). Inspired by the use of logical clocks for ordering events in distributed systems~\cite{lamportSeminalPaper, paxos_made_simple}, we introduce the notion of ``Delivery Clocks'' to overcome this issue. Corresponding to each MP, we maintain a delivery clock that tracks the progress of market data delivery to the MP. We show that \emph{ordering trades from the MP based on its delivery clock (DBO)} coupled with imposing certain \emph{restrictions on how these delivery clocks advance} (i.e., controlling the \emph{pace} of delivery of market data to MPs) can help account for delay variations in delivery of market data to MPs and enable the CES to achieve response time fairness. }

\attn{The challenge in ordering trades this way is that it is hard to measure response times since the cloud-provider does not know how the MP generated a specific trade (i.e., which data triggered the trade). Inspired by the use of logical clocks for ordering events in distributed systems~\cite{lamportSeminalPaper, paxos_made_simple}, we introduce the notion of ``Delivery Clocks'' to overcome this issue. Corresponding to each MP, we maintain a delivery clock that tracks the progress of market data delivery to the MP. We show that \emph{ordering trades from the MP based on its delivery clock (DBO)} coupled with \emph{controlling how these delivery clocks advance}\footnote{\attn{By controlling the \emph{pace} of delivery of market data to MPs}.} can help account for delay variations in delivery of market data to MPs and enable the CES to achieve response time fairness. }


%To this end, in \S\ref{s:core}, we establish the properties (for ordering trades and delivery of market data) required for achieving fairness. These properties can serve as guiding principles for building end-to-end schemes that achieve fairness (with high probability). In \S\ref{s:exp}, we use these properties to propose a few simple schemes and evaluate their performance against state-of-the-art.

\attn{To this end, in \S\ref{s:core}, we first show how DBO on its own can help improve fairness. Next, we establish some fundamental requirements on pacing of market data delivery for achieving perfect fairness. We show that if these requirements are met, DBO can indeed provide perfect fairness. In \S\ref{s:exp}, we use DBO and the constraints on pacing as our guiding principles to propose a few simple schemes and evaluate their performance.}% against state-of-the-art.}


Contrary to the current {\it modus operandi} of financial exchanges, where fairness has limited scalability and comes at a premium, our solution does not rely on equal latency between the CES and MPs and hence scales to arbitrarily sized datacenters or even across datacenters and regions. This property could be the building block for democratizing fairness in financial exchanges, with all MPs getting  equal opportunities when trading. 

%While we focus on fairness for financial exchanges, our approach is general and applicable for providing fairness in many other %distributed system settings. %where there are multiple participants taking actions based on the same real-time data from a central server. 
%Examples include, multi-player games where the game is hosted in a cloud server, advertisement auctions where multiple algorithmic bots bid on a common good, etc. %\attn{We believe that more such uses cases will emerge in future where fairness will be an important desired property.} %Going forward, logical clocks might prove to be critical in building generalized systems where any process can communicate with any other process in a fair manner.
%\pg{talk about the structure of the paper. Will write this when the rest of the paper in flushed out better.}


%We show that ordering trades from the MP based on its delivery clock can help account for delay variations in delivery of market data and enable the CES to order trades based on the response time for fairness. 

%time can be very helpful for measuring response times and ordering trades for fairness.







\if 0

Most of the major financial exchanges (such as NASDAQ, CME, NYSE) run their Central Exchange Server (CES) in  on-premise data centers. At a high level, the CES generates market data and distributes it to various market participants (MPs) in real time. Certain MPs (commonly known as high-frequency traders), rapidly react to new market data issuing a high volume of transactions: their profit is highly dependent on winning the `race for speed', aiming to submit their trade orders before other competing MPs.\footnote{High frequency traders are very aggressive in reducing latency: they often use programmable smartNICs to shave off just ns of latency on their end to gain competitive advantage.}
To accommodate fair competition based on speed of trading, financial exchanges provide 
\pg{Fairness with regards to such `reactive' trade orders constitutes simultaneous delivery of market data to the interested MPs, and processing of the trade orders based on their submission time.} Contemporary financial exchanges provide such fairness to interested MPs at a premium cost: they offer colocation services of the MPs' servers at the same datacenter with the exchange's CES, where they are able to provably guarantee equal bidirectional latency from the CES to all colocated MPs;
%The financial exchanges often go to great lengths in achieving equal bi-directional latency between the CES and the colocated MPs: 
it is not uncommon, for example, for exchanges such as NASDAQ to use equal-length cables for all colocated MPs. For the rest of the MPs -- who either do not profit from such trading strategies or cannot afford the colocation services -- fairness \pg{of such kind} is not available. Such MPs typically receive the market data stream and submit orders over variable-latency private or public WAN links.
\fi

==> outline.tex <==
\section{Outline}

\subsection{Condensed outline}
\begin{outline}
    \1 Title: Enabling fairness for traders competing on speed in  environments with unpredictable latency \radhika{perhaps too long and wordy: maybe ``Fair Trading in Environments with Unpredictable Latency'' or ``Response Time Fairness in Cloud-hosted Financial Exchanges''}
    \1 Introduction
        \2 Purpose
            \3 Why is what we are doing important
            \3 What is cool?
            \3 What are our results?
            \3 \pg{What is the selling point?}
    \1 Background and Motivation
        \2 Key points
            \3 Financial exchanges are moving to the cloud
            \3 Model of competing speed trades
            \3 How people solve it currently
            \3 Broad point Hard to provide fairness for speed trading in unequal latency environment
            \3 Insight: we can solve without actually ensuring equal delivery
            \3 One way latency model\pg{why include it}
            \3 Assumptions and Goals and Non Goals \pg{Global network.}
            \3 \pg{related work?}
    \1 Design
        \2 Key points
            \3 Strawman + challenges
                \4 \pg{Impossibility result}
            \3 DBO on its own: Talk about equal inter-delivery time. Just DBO is good.
            \3 DBO + Batching and Pacing: 
                \4  Theorem: Talk about that is the minimum property you need 
            \3 Ordering Buffer
            \3 Section on analysis, parameter setting
                \4 \pg{Trades based on different data points?}
                \4 Latency: Theoretical bound and what our system achieves
                \4 Straggler mitigation
                \4 Impact of C and delta, heartbeats
                \4 Trades > $\delta$: 
                \4 Is batching and pacing necessary.
                \4 Communication with the outside world, preventing frontrunning, other attack earliest submission
                \4 Impact of clock drift rate 
                \4 Impact of losses \pg{All loses are handled out of band. If a market data is lost, retransmitted out of band does not hit delivery clock, If a trade is lost}
                \4 Impact of RB->MP latency: \pg{Maybe say that what if RB cannot be implemented close to the MP NIC}
                \4 What if RB/OB overflows
    \1 Implementation and Practical Challenges 
        \2 Question: To what extent should we go into details on the Blue Field and the cloud implementation. 
            \3 Help from Eashan, Frank and Ilias required.
            \3 \radhika{An alternative is to split this into two sections. First one is ``practical challenges'' that tackles the question you have below on the properties you need. It could also be a more general section where you are not tying yourself to a specific implementation e.g. based on smartNICs. Perhaps some of the analysis/parameter setting points that are less theoretical and more empirical/implementation oriented can also come under this section. The following section can be the implementation section where we talk about the BlueField and the cloud implementation.}
        \2 Purpose
            \3 How do you implement OB and RB and what properties should they have. Specific Blue field implementation.
        \2 Key points to make
            \3 RB: Should be close to the MP, RB should have access to a clock and maintain the delivery clock, mark and modify packets, Hold and release packets at the specified time. Trusted RB. \pg{Is RB bump in the wire?}
            \3 OB: Handling so many heartbeats, multi-threaded operation. Trusted OV
            \3 Blue field implementation
    \1 Evaluation
        \2 Key points to make
            \3 Blue field: fix RTs, two MPs, compare Direct + DBO, DBO+LRTF, Direct delivery, + anythgin you can think of
            \3 Cloud: 10 MPs, Response Times taken from a distribution (burdisch paper https://www.bis.org/publ/work955.pdf), Show impact of heartbeats, delta and C on latency and fairness \3 Simulation: Large scale, ideal latency comparison, impact of large number of participants, straggler mitigation
    \1 Discussion
        \2 Multiple exchanges
        \2 Limitations of the compute model
        \2 Failures 
        \2 other settings where applicable
    
                 

\end{outline}

\subsection{All thoughts}


\begin{outline}
    \1 Title: Enabling fairness for traders competing on speed in  environments with unpredictable latency
    \1 Introduction
        \2 Purpose
            \3 Why is what we are doing important
            \3 What is cool?
            \3 What are our results?
    \1 Background and Motivation
        \2 Question: Should there be a separate CES for each asset class. \pg{How does this work relate to the work in the distributed systems space (talk to Lamport, Jay Lorch)} \pg{we should talk to some HFT participant. Talk about how jitter and latency differences kill competition. Ensuring latency on average is not enough. Talk about fair racing in the burdisch model.}
        \2 Purpose
            \3 Necessary background information for people to understand the problem and the challenges associated.
        \2 Key points to make (not necessarily in order)
            \3 References: Based on our discussion with three major exchanges
            \3 Background on how financial exchanges operate today, emphasis on speed based traders, and how fairness is important, talk about which data is communicated and how. (maybe a forward pointer to external streams)
            \3 Financial exchanges are considering moving to the cloud. Benefits include lower cost, ease of usage, scalability. (Minor talk about how all financial exchanges located within the same datacenter might improve things for participants [same MPs machines for different exchanges will be able to communicate with other faster]).
            \3 Unpredictable latencies make fairness or rather simultaneous delivery of data challenging
            \3 Previous solutions: clock syncronization (even with perfect clock sync we dont solve the problem, impossibility theorem on simultaneous delivery of data, high latency on average problem walk through an example? Past work on two generals problem) and financial systems based solutions. Why is replicating the current setup not possible? Why setting a deadline is hard (increases latency).
            \3 Non Goals We are not attempting to provide an answer to how networking and communication should be handled in such a scenario. We are also not going to bother which reliability of the CES and the MP machines. No mention of losses. \pg{Even in current system losses are handled out of band.}
            \3 Goals/Advantages: Provide fairness in an uncertain network environment. Overall system latency is critical. No changes to how the CES and the MPs operate. No looking at the data. Trust model: The CES cannot trust the MPs. No collusion between MP attacks possible (no front running essentially). Plug and play? While we dont care about loss recovery, losses shouldn't slow down the entire system.
            \3 Other kinds of logical clocks? Here or later?
            \3 \eg{Other use cases of RTF?}
    \1 Design
        \2 Question \pg{(flow is still unclear?), how do logical clocks fit into this stuff, Justify the compute model? What should be the definition of fairness be (ordering for two trades generated using two different points). Should we have a theorem proving the minimum bound on latency for such fairness. Maybe show equivalence of response time fairness to equal latency system.}
        \2 Key Points to make
            \3 Key Insight: Trades are not generated in isolation, look at market data and trade ordering together
                \4 Introduce the basic architecture, compute model and definition of response time fairness. Single response time, a single machine will be relaxed later. Assumptions about network.
                \4 Not all trades fit this model 1) External data streams 2) Trades generated using multiple data points
                \4 Challenges response time is not known
                \4 Definition in words, later define properly
            \3 Solution
                \4 Part 1: Simple scenario with two participants and fixed latency, how do we solve this?
                \4 terminology
                \4 Introduce DBO
                \4 Show DBO alone doesn't show when delivery times are not consistent
                \4 Define fairness and derive minimum properties for delivery times and show it works
                \4 Strong fairness, impossibility result
                \4 approximate fairness, Include S1, talk about a PID controller 
                \4 limited fairness, Include S2
                \4 How the OB works and it orders stuff, heartbeats. Latency variations on the reverse path.
            \3 Miscellaneous design concerns
                \4 Stopping front running attacks
                \4 Straggler mitigation
                \4 Impact of RB to MP latency: \pg{if we can measure can we correct it. Prbably not. HArd to maintain inter-delivery time properties. we can still quantify impacy of RB->Mp latency by assuming bounds.}
                \4 Trades generated using multiple data points. What does response time fairness mean in this case and 
                \4 Allowing external participants
                \4 Impact of clock drift rate.
    \1 Implementation and Practical Challenges 
        \2 Question: To what extent should we go into details on the Blue Field and the cloud implementation. 
            \3 Help from Eashan, Frank and Ilias required.
        \2 Purpose
            \3 How do you implement OB and RB and what properties should they have. Specific Blue field implementation.
        \2 Key points to make
            \3 RB: Should be close to the MP, RB should have access to a clock and maintain the delivery clock, mark and modify packets, Hold and release packets at the specified time. Trusted RB
            \3 OB: Handling so many heartbeats, multi-threaded operation. Trusted OV
            \3 Blue field implementation
    \1 Evaluation
        \2 Questions: \pg{Eashan and Ilias can you add here?} \pg{Handle RB->MP latency}
        \2 key points to make
            \3 Three subsections for three implementations (blue field, cloud, simulation). For each think about what kind of experiments would we and can we show. Eashan a good starting point is to think about the purpose of each one. Think about specific experiments and graphs.
                \4 BlueField. Purpose: Real hardware feasibility. Capability: Can show simple experiments with two participants. Graphs?
                \4 Cloud. Purpose: Advantage of our system in real cloud settings. I think we should do a single experiment with 5/10 participants. Graphs? Evaluate different parts of the design.
                \4 Simulations. Purpose: System working with a large number of participants. Establish micro points about our design here. Include s2 from hotnets paper here. Graphs? Some sort of optimal baseline based on a oracle? What people use simulations for: 1) Scale 2) Sensitivity Analysis 3) Insights (Impact of various parts of design e.g., heart beat duration, comparison with some sort of an oracle scheme, break down of latency on our system, impact of delta and C on the latency distribution of the system).
            \3 Evaluation metrics
        \2 Graphs: Trying to answer why use our system (better fairness numbers) and what the limitations are (latency in large-scale experiment). Trust issues resolved by hardware implementation.
            \3 Simulation: start with simulation heatmaps from HotNets paper showing improved fairness numbers for our schemes. Cover all new schemes we are proposing against Cloudex and direct data delivery. Skip latency numbers. Run with only 2 MPs.
            \3 Cloud: Run a single experiment with 5-10 MPs. Skip fairness numbers.
                \4 Show End-to-End latency (from generation to trade being forwarded to ME minus response time) over time for one MP. Run setup for 10min. We could add lines for all schemes on one graph. Can be used to show regions of spikes where we had stragglers/latency spikes. Additionally shows stability of schemes.
                \4 Show the CDF of above graph. Shows how much additional latency is introduced by our schemes in general over other schemes.
            \3 Bluefield: 
                \4 Compare DBO to the ideal fairness number. Run experiment by sampling Response time from a distribution. Get ideal response time fairness number and get fairness number due to various schemes. Show bar graph for a pair of MPs.
                \4 Show end-to-end latency graph for 1 MP and compare with cloud. Shows any performance change against cloud.
            \3 Others?:
                \4 Study about RB to MP latency - compare latency and fairness numbers between Bluefield and Cloud implementation.
                \4 Show fairness numbers in Cloud implementation?
                \4 Show how, on changing hyperparameters, performance changes. (end-to-end latency over time and fairness).
    \1 Discussion and Limitation
        \2 Purpose
            \3 Answer Potential questions a reviewer might have
            \3 Future directions
        \2 Key Points to make
            \3 Fundamental limitation slowest network latency slows down the entire system. \pg{Discuss tradeoff our system offers?}
            \3 RB OB failure
            \3 Limitations of the compute model
            \3 Impact of other streams such as news
            \3 Other considerations: Multicast, HPC cluster, reliability, etc.
            \3 Multi exchange scenario, multiple sources of information
            \3 Multi cloud scenario
            \3 Other metrics of fairness: Resource Fairness
            \3 Other settings where this is applicable
            \3 Speculative execution to leave out particcipants that are not placing trades.
    \1 \pg{Concerns raised by HotNets Reviewers}
        \2 Impact of RB->MP latency
            \3 Answer: We are at the NIC, Boundaru of MP is the NIC. Additionally analyse the impact of RB->MP latency in our system.
        \2 Why would exchanges move to the cloud
            \3 Answer: Its already happening. Talk about the partnerships that already happened.
        \2 Collusion attacks.
            \3 Answer: Have a specific sub section
        \2 External streams of market data
            \3 There are much more infrequent events. Fairness w.r.t. such streams is not required.
        \2 Writing and Notation is complicated
            \3 Answer: Explain in words to the extent possible. Ask Radhika.
\end{outline}
